HyperDynamics: Meta-Learning Object and Agent Dynamics with Hypernetworks

We propose HyperDynamics, a dynamics meta-learning framework that conditions on an agent's interactions with the environment and optionally its visual observations, and generates the parameters of neural dynamics models based on inferred properties of the dynamical system. Physical and visual properties of the environment that are not part of the low-dimensional state yet affect its temporal dynamics are inferred from the interaction history and visual observations, and are implicitly captured in the generated parameters. We test HyperDynamics on a set of object pushing and locomotion tasks. It outperforms existing dynamics models in the literature that adapt to environment variations by learning dynamics over high dimensional visual observations, capturing the interactions of the agent in recurrent state representations, or using gradient-based meta-optimization. We also show our method matches the performance of an ensemble of separately trained experts, while also being able to generalize well to unseen environment variations at test time. We attribute its good performance to the multiplicative interactions between the inferred system properties -- captured in the generated parameters -- and the low-dimensional state representation of the dynamical system.

==> 1_abstract.tex <==

\begin{abstract}
\todo{i learnt we need to be positive as opposed to negative in abstract+intro}

Humans build dynamics models to predict how the environment responds to their actions. 
They adapt  these models on-the-fly during interactions with the environment,  if the  actual outcomes deviate from their  predictions. 
We propose HyperDynamics (HD), a model that conditions on the history of interactions of the agent with the environment and visual observations to generate  parameters for   neural models that reflect dynamics of the agent and its environment. The generated dynamical models  operate over instantaneous (non-recurrent) low-dimensional state representations of the agent and its environment, such as the agent's joint configuration and 3D object locations. 
We test HD on  tasks of ... . We show superior performance over existing approaches that incorporate interaction history using recurrent state representations or through meta-learning gradient based optimization. We test HD on the visual task of pushing objects and outperform formulations that learn dynamics directly over high-dimensional 2D images or 3D visual features maps. HD propose a new way of incorporate interactions and visual information, by generating the "expert" low-dimensional dynamics model, and thus can both adapt across physical and visual properties of different systems, while benefiting from the low-dimensionality of the state parametrization. 
%We attribute the superior performance of HD to the multiplicative way of the history interaction  and visual context with the low-dimensional state representation of the environment and the agent. 
\end{abstract}



\begin{comment}


%Model-based reinforcement learning and planning methods resemble this mechanism.
%However, many contemporary methods assume a single system with fixed properties and learn a dedicated model (i.e., an \textit{expert}) for that system, resulting in failures when the system behavior changes.
This limitation can be addressed by training separate experts for each dynamical system and using them accordingly.
However, this often becomes impractically computationally expensive as the number of systems grows, and also makes it impossible to adapt to new systems that were not encountered during training.
Other existing approaches feed system features directly as input to a global dynamics network, with the hope of transferring acquired knowledge to unseen systems.
We propose \textit{HyperDynamics}, a framework that enables models to effectively condition on system properties, by generating a separate expert for each system on the fly.
Specifically, we evaluate our approach in an object pushing setting.
In this setting, HyperDynamics networks use an object's appearance and its response to a few interactions to generate the parameters of a dynamics network dedicated to the observed object.
We show that this method is able to match the performance of an ensemble of object-specific experts, while also being able to generalize well to unseen objects with novel properties.
Finally, we also show that the proposed method outperforms alternative formulations that directly take object features as input to the dynamics network.

\end{comment}

==> 1_abstract_2.tex <==

\begin{abstract}



Humans build models to predict how the world behaves and use them to plan actions and achieve intended goals.
Model-based reinforcement learning and planning methods resemble this mechanism.
However, many contemporary methods assume a single system with fixed properties and learn a dedicated model (i.e., an \textit{expert}) for that system, resulting in failures when the system behavior changes.
This limitation can be addressed by training separate experts for each dynamical system and using them accordingly.
However, this often becomes impractically computationally expensive as the number of systems grows, and also makes it impossible to adapt to new systems that were not encountered during training.
Other existing approaches feed system features directly as input to a global dynamics network, with the hope of transferring acquired knowledge to unseen systems.
We propose \textit{HyperDynamics}, a framework that enables models to effectively condition on system properties, by generating a separate expert for each system on the fly.
Specifically, we evaluate our approach in an object pushing setting.
In this setting, HyperDynamics networks use an object's appearance and its response to a few interactions to generate the parameters of a dynamics network dedicated to the observed object.
We show that this method is able to match the performance of an ensemble of object-specific experts, while also being able to generalize well to unseen objects with novel properties.
Finally, we also show that the proposed method outperforms alternative formulations that directly take object features as input to the dynamics network.

\end{abstract}





==> 1_abstract_xian.tex <==
\begin{abstract}
Humans build models to predict how the environment responds to their actions, and adapt these models on-the-fly during interactions with the environment. %,  if the  actual outcomes deviate from their predictions.   
We propose HyperDynamics, a framework that conditions on an agent's past interactions with the environment and/or its visual observations, and generate the parameters of an action-conditioned  dynamics model based on inferred system properties. Such generated models serve as \textit{experts} that work specifically for the dynamical system at present, and operate over instantaneous low-dimensional state representations of the agent and its environment. 
We test HyperDynamics on a set of object pushing and locomotion tasks. Our proposed method outperforms models that learn dynamics over high dimensional visual state representations, recurrent dynamics  models,  or gradient-based meta-learning models. We also show our method matches the performance of an ensemble of separately trained experts, while also being able to generalize well to unseen environment variations. We attribute its performance gain to our multiplicative way of combining explicit factorization of system features with the low-dimensional state representations of the system.
\end{abstract}



==> 2_intro.tex <==
\section{Introduction} \label{sec:intro}

Humans learn dynamics models that predict results of their interactions with the environment, and use their models' predictions for selecting actions to achieve intended goals \cite{Miall:1996:FMP:246663.246676,NIPS1998_1585}.  
These models capture intuitive physics and mechanics of the world 
 and are remarkably versatile: they are  expressive and can be applied to all kinds of environments that we encounter in our daily lives, that may wildly vary in their physical  properties and visual appearance.   
In addition, humans do not consider these models fixed over the course of interaction; we observe how objects behave
and quickly adapt our model for the situation in hand based on new observations. 
Let us consider the scenario of moving an object on the ground. We can infer how heavy the object is by simply looking at it, and we can
then decide how hard to push. If it does not move as expected, we might realize it is heavier than we thought and increase the force we apply \cite{hamrick2011internal}.



 
 
Motivated by this, we propose {\em HyperDynamics}, a model that  generates parameters for low-dimensional dynamics models (experts)  based on observations of how the environment behaves. HyperDynamics has two modules: i) a hypernetwork \cite{ha2016hypernetworks} that conditions on a few  agent-environment interactions and visual object appearance and generates parameters of a dynamics model dedicated to the observed system, and ii) a target dynamics model whose parameters are generated  that takes as input the current system state (agent configuration and 3D object locations) and the agent action, and predicts the next system state, as shown in Figure \ref{fig:overview}. The hypernetwork then takes the predicted state as input, and can optionally generate a new target dynamics model, adapted to the predicted states and visual appearances of the environment.  We will be referring to this target dynamics model as an expert, as it specializes on encoding the dynamics of a particular scene at a certain point in time, and cannot generalize across scenes.  
  HyperDynamics are trained in an end-to-end differentiable manner to minimize state prediction of the target generated networks in each task.



HyperDynamics learn a mapping between  how a scene looks and behaves to its low-dimensional dynamics function,  i.e., the mapping from states and actions $(s_t,a_t)$ to the next states $s_{t+1}$ or next state difference $\delta s_{t+1}$, where the state contains only fast changing---such as agent and object 3D or 2D locations. 
 Similar systems will have similar corresponding dynamics functions. HyperDynamics attempt to exploit this regularity and learn such commonalities across different systems, or within the same system across different timesteps. 
 
 
 To place  HyperDynamics in the context of existing  literature on model learning and adaptation, we distinguish  four  groups of methods, depending on  whether they explicitly distinguish between  dynamic---such as agent and object 3D or 2D locations and poses---and static ---such as mass, inertia, 3D object shape---properties of the system,  whether they update the dynamics model parameters or  the static property values in the course of interaction, and  whether they consider visual sensory input  or operate on a predefined low-dimensional state representation. 
 Though such exposition may not be exhaustive, it will help us put the proposed work in perspective with existing methods. 
 
 
 \textbf{(i)} No adaptation.  These methods concern  dynamics model over low-dimensional states of the system,  developed or learned for a specific system and cannot generalize across different  physical properties of the same system,  or across different systems \cite{}. 
Such expert dynamics models are popular formulations in the literature. 
As a matter of fact, it's been shown recently that modelling epistemic and aleatoric uncertainty of such expert models during forward unrolling permits  model-based formulations to surpass  model-free RL (in manipulating a single object or controlling a single system) both in low- and high-data regimes \cite{NIPS2018_7725}. 



%\textbf{(i)} Mixture of experts  \cite{}. These methods maintain a pool of dynamical models,  each developed or learned for a specific system, and select the fittest one at test time  using few interactions and Bayesian optimization. % to balance. 


\textbf{(ii)} Visual dynamics and self-supervision \cite{}. 
%In this group, we consider  dynamics model over low-dimensional states of the system,  developed or learned for a specific system and cannot generalize across different  physical properties of the same system,  or across different systems, and  b)
These methods learn dynamics model over high-dimensional sensory observations, such as images or 3D pointclouds \cite{}, that  predict a representation for the sensory input for the next time step. They expect the physical properties of the system to be discerned through the history of sensory observations. When the methods can be self-supervised by future frame prediction \cite{densephysnet, DBLP:journals/corr/FinnGL16,DBLP:journals/corr/FinnL16,ebert2018visual,actionconditioned,DBLP:journals/corr/abs-1710-05268,NIPS2015_5859,DBLP:journals/corr/abs-1903-00374}, they can be adapted through gradient descent at any test system, yet that would require a large number of interactions. 
%daptation through self-supervision  \cite{densephysnet, DBLP:journals/corr/FinnGL16,DBLP:journals/corr/FinnL16,ebert2018visual,actionconditioned,DBLP:journals/corr/abs-1710-05268,NIPS2015_5859,DBLP:journals/corr/abs-1903-00374}





 \textbf{(iii)} System identification \cite{conf/eccv/BhatSP02}. These methods model explicitly the static properties of the dynamical system  using a small set of semantically meaningful physics parameters, such as mass, inertia, .... \cite{ajay,mrowca2018flexible}, %that are hard to discern visually. 
 and  adapt by learning their values  from data on-the-fly  \cite{chen2018hardware, li2018learning,  sanchez2018graph, battaglia2016interaction,pmlr-v80-sanchez-gonzalez18a,}. 
 %\todo{we need 4-5 traditional robotics works here that use Newtonian equations}. 
 %This process has been used both with Newtonian system of equations of motion, as well as learning-based dynamic  models, such as MLPs \cite{} or graph neural networks \cite{battaglia2016interaction, li2018learning}. 


\textbf{(iv)} Recurrent state representations \cite{pushnet}. These models learn to predict the next state from a history of state-action interaction  $s_{t+1}=f(s_{t-k},a_{t-k},...s_{t-1},a_{t-1};\phi)$, and 
%They do not explicitly separate static and dynamic properties of the system, and 
the recurrent hidden state implicitly captures information regarding the physical properties of the system. 


%\textbf{(iii)} Model learning and adaptation through self-supervision  \cite{densephysnet, DBLP:journals/corr/FinnGL16,DBLP:journals/corr/FinnL16,ebert2018visual,actionconditioned,DBLP:journals/corr/abs-1710-05268,NIPS2015_5859,DBLP:journals/corr/abs-1903-00374}.
%These methods adapt the dynamics model on the fly by finetuning it at test time \cite{ijcai2018-369}.
%However, this can cause overfitting to the history of interactions if the model capacity is high, and has been used effectively with low-dimensional local models \cite{fu}.

\textbf{(v)} Online model adaptation through meta-learning gradient descent optimization \citep{DBLP:journals/corr/FinnAL17,Nagabandi2019LearningTA, clavera, DOMe}. These methods consider dynamics models and adapt all their parameters (as opposed to a small set of physic properties) through gradient descent. The model is optimized so that few gradient steps will generate a model that can perform well in the test scenario, as opposed to overfiting to the small set of interactions, by backpropagating through the gradient descent optimization process.  




HyperDynamics adapts all model's parameters based on interaction history and visual context, similar to methods in ((i),(ii)) but it generates  parameters for the dynamics model through a hypernetwork as opposed to gradient based optimization. The low-dimensional state representation of the generated target dynamics model only captures fast changing dynamic state, similar to methods in (). Static properties are not explicitly represented rather implicitly inferred through conditioning on recent history of interactions, like recurrent models in (), It can condition on high-dimensional visual information as in the object-centric models of \cite{}. Specifically, we use a 3D object detector  to localize the object in 3D and feed its 3D feature map to the hypernetwork to generate parameters for a dynamics model that operates over the 3D object location and agent configuration and predicts future 3D object location and orientation, and 3D agent's configuration.  Then, the 3D feature map is oriented to predict the parameters of the model in the next timestep.  
 The only difference is that instead of directly optimizing the weights of such expert dynamics models \cite{NIPS2018_7725}, we will be predicting them using a hypernetwork. %Our model is trained by back-propagating the expert model's prediction error in an end-to-end differentiable manner.


We evaluate HyperDynamics on single- and multi-step state prediction, as well as  downstream model-based planning and control tasks.  Specifically, we apply it in the tasks of.  and compare with representative models from categories I,ii,iv and iv, showing superior performance. We further evaluate HyperDynamics in the visual task of  pushing diverse objects to different locations on the table surface, and compare against representative models in i,ii, showing better generalization to novel objects and camera viewpoints. 
To the best of our knowledge, this is the first work that considers hypernetworks for adapting dynamics models. We show through exhaustive ablations the benefits of the proposed methods, which we attribute to the multiplicative way of the history interaction  and visual context with the low-dimensional state representation of the environment and the agent. We further discuss implementation details that were crucial in getting the hypernetwork neural generation to work robustly, and we will share our datasets and code to stimulate research in this direction. 



==> 2_intro_iclr.tex <==
\section{Introduction} \label{sec:intro}

Humans learn dynamics models that predict results of their interactions with the environment, and use such predictions for selecting actions to achieve intended goals \citep{Miall:1996:FMP:246663.246676,NIPS1998_1585}.  
These models capture intuitive physics and mechanics of the world and are remarkably versatile: they are  expressive and can be applied to all kinds of environments that we encounter in our daily lives,  with varying dynamics and diverse visual and physical properties.  
In addition, humans do not consider these models fixed over the course of interaction; we observe how the environment behaves in response to our actions
and quickly adapt our model for the situation at hand based on new observations. 
Let us consider the scenario of moving an object on the ground. We can infer how heavy the object is by simply looking at it, and we can
then decide how hard to push. If it does not move as much as expected, we might realize it is heavier than we thought and increase the force we apply \citep{hamrick2011internal}.

Motivated by this, we propose {\em \HD}, a framework that  generates parameters for dynamics models (experts) dedicated to the situation at hand, based on observations of how the environment behaves. HyperDynamics has three main modules: i) an encoding module that encodes a few agent-environment interactions and the agent's visual observations into a latent feature code, which captures the properties of the dynamical system, ii) a hypernetwork \citep{ha2016hypernetworks} that conditions on the latent feature code and generates parameters of a dynamics model dedicated to the observed system, and iii) a target dynamics model constructed using the generated parameters that takes as input the current low-dimensional system state and the agent action, and predicts the next system state, as shown in Figure \ref{fig:overview}.   We will be referring to this target dynamics model as an \textit{expert}, as it specializes on encoding the dynamics of a particular scene at a certain point in time.  \HD\ conditions on real-time observations and generates dedicated expert models on the fly. It can be trained in an end-to-end differentiable manner to minimize state prediction error of the generated experts in each task. 


\begin{figure*}[t]
\centering
		\includegraphics[width=0.8\textwidth]{figures/arch.png}
		\caption{\HD\ encodes the visual observations and a set of agent-environment interactions and generates the parameters of a  dynamics model dedicated to the current environment and timestep using a hypernetwork. \HD\ for pushing follows the general formulation, with a visual encoder for detecting the object in 3D  and encoding its shape, and an interaction encoder for encoding a small history of interactions of the agent with the environment.
		}
			\label{fig:overview}
			\vspace{-4ex}
\end{figure*}

 
 
 To place  HyperDynamics in the context of existing  literature on model learning and adaptation, we distinguish  four  groups of methods, depending on  whether they explicitly distinguish between  dynamic---such as joint configurations of an agent or poses of objects being manipulated---and static ---such as mass, inertia, 3D object shape---properties of the system, and whether they update the dynamics model parameters or  the static property values of the system. 
 Though such exposition may not be exhaustive, it will help us put the proposed work in perspective with existing methods. 
 
 
 \textbf{(i)} No adaptation.  These methods concern  dynamics model over either low-dimensional states or high-dimensional visual inputs of a specific system,  without considering  potential changes in the underlying dynamics. These models tend to fail  when the system behavior changes. 
Such \textit{expert} dynamics models are popular formulations in the literature \citep{watter2015embed, banijamali2018robust, Fragkiadaki2015LearningVP,   zhang2019solar}. They can be adapted through gradient descent at any test system, yet that would require a large number of interactions. 


\textbf{(ii)} Visual dynamics and recurrent state representations. These methods operate over high-dimensional visual observations of systems with a variety of properties \citep{DBLP:journals/corr/FinnL16, ebert2018visual, li2018push,xu2019densephysnet,DBLP:journals/corr/MathieuCL15, actionconditioned,DBLP:journals/corr/PathakAED17}, hoping the visual inputs could capture both the state and properties of the system. Some also attempt to encode a history of interactions with a recurrent hidden state \citep{densephysnet,li2018push, ebert2018visual, sanchez2018graph, hafner2019planet}, in order to implicitly capture information regarding the physical properties of the system. These methods use a single and fixed global
dynamics model that takes system properties as input directly, together with its state and action.

 \textbf{(iii)} System identification \citep{conf/eccv/BhatSP02}. These methods model explicitly the properties of the dynamical system using a small set of semantically meaningful physics parameters, such as mass, inertia, damping, etc. \citep{ajay,mrowca2018flexible}, and adapt by learning their values  from data on-the-fly  \citep{chen2018hardware, li2018learning,  sanchez2018graph, battaglia2016interaction,pmlr-v80-sanchez-gonzalez18a}. 


\textbf{(iv)} Online model adaptation via meta-learning \citep{DBLP:journals/corr/FinnAL17,Nagabandi2019LearningTA, clavera, DOMe}. These methods perform online adaptation on the parameters of the dynamics models through gradient descent. They are optimized to produce a good parameter initialization that can be adapted to the local context with only a few gradient steps at test time.


The expert models in (i) work well for their corresponding systems but fail to handle system variations. A natural solution to address this is to train a separate expert for each dynamical system. However, this can hardly scale and doesn't transfer to systems with novel properties. Inspired by this need, \HD\ aims to infer a system's properties by simply observing how it behaves, and automatically generate an expert model that is dedicated to the observed system. Methods in (ii) and (iii), though attempting to infer system properties, optimize a single and fixed global dynamics model, which takes as input both static system properties and fast-changing states, with the hope that such a model can handle variations of systems and generalizes. We argue that a representation which encodes system information varies across different system variations, and each instance of this presentation ideally should correspond to a different dynamics model that needs to be used in the corresponding setting. These models are different, but also share a lot of information as similar systems will have similar dynamics functions. \HD\ makes explicit assumptions about the relationships between these systems, and attempts to exploit this regularity and learn such commonalities across different system variations.


We evaluate HyperDynamics on single- and multi-step state predictions, as well as  downstream model-based control tasks.  Specifically, we apply it in a series  of object pushing and locomotion tasks. Our experiments show that \HD\ is able to generate performant dynamics models that match the performance of separately and directly trained experts, while also enabling effective generalization to systems with novel properties in a few-shot manner, outperforming representative models from the categories discussed above. We attribute its performance gain to the multiplicative way of combining explicit factorization of encoded system features with the low-dimensional state representation of the system. Our code is included in the supplementary material.
\vspace{-1ex}


==> 2_intro_xian_final.tex <==
\section{Introduction} \label{sec:intro}

When humans manipulate objects or interact with the world, they can generally predict how the world will change as a result of their actions.
Such predictions are possible thanks to the multiple models of the world's dynamics that the human brain possesses, which are learnt and continuously updated based on our experiences \citep{ha2018worldmodels}.
These {\em world models} are remarkably versatile: they are very expressive and can be applied to all kinds of systems that we encounter in our daily lives, with varying dynamics and diverse visual and physical properties.  
In addition, they are not fixed over the course of interaction; we observe how objects behave
and quickly adapt our models based on new observations. 
Let us consider the scenario of moving an object on the ground. We can infer how heavy the object is by simply looking at it, and we can
then decide how hard to push. If it does not move as expected, we might realize it is heavier than we thought and increase the force we apply.

World models enable humans to plan actions in order to achieve intended goals. The fields of model-based reinforcement learning (MBRL) and  trajectory optimization resemble this  mechanism of model-predictive action selection. They focus on developing models that predict the next state of a dynamical system given its current state and an agent action. These models are then unrolled forward in time for evaluating and choosing action sequences that achieve long term goals. However, many contemporary model-based approaches assume a fixed system without considering potential change in the underlying dynamics, and train a fixed dynamics model \cite{watter2015embed, banijamali2018robust, Fragkiadaki2015LearningVP,   zhang2019solar}. Such \textit{expert} models tend to fail when the system behavior changes. A natural solution to address this is to train a separate expert for each dynamical system. However, this can hardly scale with the  number of systems, and is not able to transfer to system with novel properties. So we  wonder, can we automatically generate an expert on the fly, by simply observing how a system behaves? Meanwhile, can such capability of \textit{generating experts} generalize to systems with novel properties not encountered during training?

Acquiring expressive and generalizable dynamics models has turned out to be a notoriously hard problem. Most prior works in this area propose methods that condition on system properties \cite{chen2018hardware, li2018learning, sanchez2018graph}, especially in the context of modeling  interactions with objects \cite{DBLP:journals/corr/FinnL16,agrawal2016learning, li2018push,xu2019densephysnet, battaglia2016interaction}, with the hope that the learned model  can transfer to novel systems. However,  many approaches use low-dimensional engineered state representations (such as explicit or estimated pose, mass and friction) \cite{chen2018hardware, li2018learning,  sanchez2018graph, battaglia2016interaction}, bypassing  high-dimensional visual input. These models cannot generalize across environments since the visual properties of the system are not taken into account. 
 Other methods condition on visual inputs, and pass system information and states directly into a single dynamics model \cite{li2018push, xu2019densephysnet, DBLP:journals/corr/FinnL16, agrawal2016learning}, with the hope that it can handle varying system properties and transfer  acquired knowledge to  novel  systems. We argue that the way these models incorporate the additional system information that encodes system properties are inefficient. Specifically, this information is a representation of the system properties that may vary across different settings, and each instance of this representation ideally should correspond to a different dynamics model---an {\em expert}---that needs to be used in the corresponding setting. 
The experts themselves can be simple models; each of them is a dynamics model targeted at a single fixed system.
However, they share a lot of information as similar systems will have similar corresponding experts. Prior work does not explicitly consider this ``local'' structure and instead attempts to learn a single global model that receives the system features as an additional input. If such a model is trained on a small number of systems, it cannot generalize well to new ones because it does not make any explicit assumptions about the relationships between these systems.

To this end, we propose {\em HyperDynamics}, a general  framework that extends the current family of model-based RL methods by enhancing them with the capability of {\em automatically generating experts} based on observations of how the system behaves.
Given a system with certain properties, HyperDynamics networks observe its visual appearance and response to a few interactions, and automatically generate parameters of a dynamics model dedicated to the observed system. This dynamics model then takes as input the current system state and the agent action, and predicts the next system state.
We evaluate HyperDynamics in the context of modeling object pushing. Specifically, we evaluate its performance for single- and multi-step motion prediction, as well as for using the learned model for downstream planning and control tasks. 
Our experiments show that with only a handful of distinct objects used for training, HyperDynamics is able to match the performance of separately and directly trained experts, while also enabling effective generalization to objects with novel properties in a few-shot manner, addressing the aforementioned limitations of existing approaches.
Note that, even though we only consider the setting of object pushing in the scope of this paper, the proposed HyperDynamics framework is general and \textit{potentially} applicable to a wide range of dynamics learning tasks, as we discuss in Section \ref{sec:conclusion}.
We hope this work marks the first step in using the idea of {\em automatic expert generation} for dynamics learning, and we leave further experimental studies on  tasks other than object pushing as an interesting direction for future work.

In summary, the main contribution of this work is that we propose a general framework that is able to generate  expert dynamics models on the fly, conditioned on system features, and apply it to  the context of object pushing.
We show that our approach matches performance of separately and directly trained experts, while also being able to transfer well to novel objects.
In addition, we also show that our model outperforms alternative formulations which feed object features (both visual and physical properties) directly into a global dynamics model, as what most prior works do. Our code and datasets will be made publicly available upon publication.


==> 3_related.tex <==
\section{Related Work}
\label{sec:related}



\paragraph{Model learning and model adaptation}
Learning dynamics  models that can generalise across environment physical and visual variations  is an open research problem whose solution would revolutionize model-based reinforcement learning, the field that investigates action selection by temporal unrolling of dynamics \cite{robotcontrol}. 
%Learning models of dynamics is a central research problem in machine learning and control. 
The difficulty of traditional analytical models to capture the complexity of real world systems \cite{} has led many researchers to pursue learning-based models of dynamics \citep{watter2015embed, banijamali2018robust, hafner2019planet, zhang2019solar}, or combine such models with analytic ones \citep{zeng2019tossingbot,ajay}. 
Dynamic models that operate over high-dimensional images are often self-supervised (no need for annotation of the state) by predicting future frames. These  methods infer a low-dimensional state of the system  from a history of 2D images or 3D poinclouds \cite{li2018push, xu2019densephysnet, DBLP:journals/corr/FinnL16, agrawal2016learning} and predict a representation for the sensory input for the next time step,  such as a future 2D image \cite{DBLP:journals/corr/FinnGL16,DBLP:journals/corr/FinnL16,ebert2018visual,actionconditioned,DBLP:journals/corr/abs-1710-05268,NIPS2015_5859,DBLP:journals/corr/abs-1903-00374}, image embedding from which an image will be reconstructed \cite{hafner2019planet}. Models that factorize images into objects or particles in 2D or 3D and estimate their dynamics using relational biases implemented through graph message passing algorithms  are harder to supervised since they need annotations regarding the objects in the scene and their trajectories over time. 
%object 2D locations from which a future image can be rendered \cite{DBLP:journals/corr/abs-1812-10972,Fragkiadaki2015LearningVP}. In the state inferred there is no explicit separation of static and dynamic properties. 
% to help the latter fight under-modeling and improve generalization.
%Many works do not consider potential change in the underlying dynamics \cite{watter2015embed, banijamali2018robust, Fragkiadaki2015LearningVP,   zhang2019solar, hafner2019planet}, resulting in potential model in case of any changes in the system behavior. In order to account for varying dynamics, various approaches propose to learn dynamics models conditioning on system properties \cite{chen2018hardware, li2018learning, graphnet}. In the context of modeling interactions with objects, many works condition on 2D visual inputs \cite{DBLP:journals/corr/FinnL16,agrawal2016learning, li2018push,xu2019densephysnet, battaglia2016interaction}, hoping that the visual inputs capture both the state and properties of the system. This includes methods that predict dynamics in a 2D image space, such as future visual frames \citep{DBLP:journals/corr/MathieuCL15,actionconditioned,DBLP:journals/corr/FinnGL16,DBLP:journals/corr/abs-1812-00568}, neural encodings of future frames \citep{DBLP:journals/corr/abs-1803-10122,DBLP:journals/corr/ChiappaRWM17,hafner2019planet,agrawal2016learning,DBLP:journals/corr/PathakAED17}, object 2D motion trajectories \citep{Fragkiadaki2015LearningVP,DBLP:journals/corr/BattagliaPLRK16,DBLP:journals/corr/ChangUTT16}, and 2D pixel motion fields \citep{DBLP:journals/corr/FinnL16,DBLP:journals/corr/abs-1710-05268,DBLP:journals/corr/FinnGL16,SE3-Nets}.
%The last two sets of methods provide future visual observations during model unrolling by warping image pixels to generate future visual observations, and feed them into their model.
%These methods use a single global model that takes system properties as input directly, together with its state and actions given by the agent. 
To infer physical properties of the system that can not be discerned from visual features, some works propose to encode a history of agent interactions  \cite{pushnet, densephysnet}.
%For expressive dynamics models represented as neural networks, online adaptation via finetuning starting from some initial set of parameters is also explored. These approaches usually require many samples and multiple passes over the data to arrive at a sensible solution \citep{ijcai2018-369}.
The meta-learning methods of dynamics in \citep{DBLP:journals/corr/FinnAL17,Nagabandi2019LearningTA,clavera} learn a parameter initialization for a dynamics model that can best be adapted through gradient descent to the system properties in hand, by backpropagating through the optimization process. The idea of using multiple model initializations for efficient adaptation to novel test conditions are investigated in \citep{adaptanimals,DOMe}.
\citet{kaushik2020fast} proposes dynamics models that alongside a state and action condition (through concatenation) on a situation embedding, which is jointly trained with a dynamics model. 

%We compare Hyperdynamics with 

has been used effectively with low-dimensional local models \cite{fu}

%in inverstigate how to use gradient based optimization so that  with the objective of learnign the dynamics of the test system as opposed 
%For example, model agnostic meta-learning (MAML) \citep{DBLP:journals/corr/FinnAL17,Nagabandi2019LearningTA,clavera} learns a parameter initialization for a dynamics model which ought to generate a well adapted dynamics model with only a few interactions at test time.
%Under diverse dynamic environments without some obvious similarity between them such an initialization learning approach has been found to require many samples to adapt effectively \citep{kaushik2020fast,DOMe}. The idea of using multiple model initializations for efficient adaptation to novel test conditions are investigated in \citep{adaptanimals,DOMe}.
%\citet{kaushik2020fast} proposes dynamics models that alongside a state and action condition (through concatenation) on a situation embedding, which is jointly trained with a dynamics model.

\paragraph{Hyper-networks}
Central to HyperDynamics is the notion of using one network to generate the parameters of another network. 
This idea has previously been studied in various domains including image classification \citep{ha2016hypernetworks}, generative models \citep{ratzlaff2019hypergan}, and neural machine translation \citep{ha2016hypernetworks,platanios2018contextual}.
These works are motivated by various intuitions, such as using the structural features of the original network to generate network layers for reduction in the number of parameters \citep{ha2016hypernetworks}, generating an ensemble of networks for the same task to improve robustness to adversarial data \citep{ratzlaff2019hypergan}, or generating language encoders conditioned on the language context for better weight sharing across languages in a machine translation setting \citep{platanios2018contextual}.
To the best of our knowledge, this is the first work that applies the idea of generating model parameters to the domain of model-based RL, and proposes to generate expert models conditioned on system properties.


==> 3_related_xian_final.tex <==
\section{Related Work}
\label{sec:related}

Learning models of dynamics is a central research problem in machine learning and control. 
The inability of traditional analytical systems to capture the complexity of real world systems has led many researchers to pursue learning-based models of dynamics \citep{watter2015embed, banijamali2018robust, hafner2019planet, zhang2019solar}, or combine such models with analytic ones \citep{zeng2019tossingbot,ajay} to help the latter fight under-modeling and improve generalization. 
Many works do not consider potential change in the underlying dynamics \cite{watter2015embed, banijamali2018robust, Fragkiadaki2015LearningVP,   zhang2019solar, hafner2019planet}, resulting in potential model in case of any changes in the system behavior. In order to account for varying dynamics, various approaches propose to learn dynamics models conditioning on system properties \cite{chen2018hardware, li2018learning, graphnet}. In the context of modeling interactions with objects, many works condition on 2D visual inputs \cite{DBLP:journals/corr/FinnL16,agrawal2016learning, li2018push,xu2019densephysnet, battaglia2016interaction}, hoping that the visual inputs capture both the state and properties of the system. This includes methods that predict dynamics in a 2D image space, such as future visual frames \citep{DBLP:journals/corr/MathieuCL15,actionconditioned,DBLP:journals/corr/FinnGL16,DBLP:journals/corr/abs-1812-00568}, neural encodings of future frames \citep{DBLP:journals/corr/abs-1803-10122,DBLP:journals/corr/ChiappaRWM17,hafner2019planet,agrawal2016learning,DBLP:journals/corr/PathakAED17}, object 2D motion trajectories \citep{Fragkiadaki2015LearningVP,DBLP:journals/corr/BattagliaPLRK16,DBLP:journals/corr/ChangUTT16}, and 2D pixel motion fields \citep{DBLP:journals/corr/FinnL16,DBLP:journals/corr/abs-1710-05268,DBLP:journals/corr/FinnGL16,SE3-Nets}.
%The last two sets of methods provide future visual observations during model unrolling by warping image pixels to generate future visual observations, and feed them into their model.
These methods use a single global model that takes system properties as input directly, together with its state and actions given by the agent. To infer implicit properties that can not be inferred from visual features, some works propose to encode a history of interactions with objects to infer their physics properties \cite{pushnet, densephysnet}.

For expressive dynamics models represented as neural networks, online adaptation via finetuning starting from some initial set of parameters is also explored. These approaches usually require many samples and multiple passes over the data to arrive at a sensible solution \citep{ijcai2018-369}.
For example, model agnostic meta-learning (MAML) \citep{DBLP:journals/corr/FinnAL17,Nagabandi2019LearningTA,clavera} learns a parameter initialization for a dynamics model which ought to generate a well adapted dynamics model with only a few interactions at test time.
Under diverse dynamic environments without some obvious similarity between them such an initialization learning approach has been found to require many samples to adapt effectively \citep{kaushik2020fast,DOMe}. The idea of using multiple model initializations for efficient adaptation to novel test conditions are investigated in \citep{adaptanimals,DOMe}.
\citet{kaushik2020fast} proposes dynamics models that alongside a state and action condition (through concatenation) on a situation embedding, which is jointly trained with a dynamics model.


Finally, central to HyperDynamics is the notion of using one network to generate the parameters of another network.
This idea has previously been studied in various domains including image classification \citep{ha2016hypernetworks}, generative models \citep{ratzlaff2019hypergan}, and neural machine translation \citep{ha2016hypernetworks,platanios2018contextual}.
These works are motivated by various intuitions, such as using the structural features of the original network to generate network layers for reduction in the number of parameters \citep{ha2016hypernetworks}, generating an ensemble of networks for the same task to improve robustness to adversarial data \citep{ratzlaff2019hypergan}, or generating language encoders conditioned on the language context for better weight sharing across languages in a machine translation setting \citep{platanios2018contextual}.
To the best of our knowledge, this is the first work that applies the idea of generating model parameters to the domain of model-based RL, and proposes to generate expert models conditioned on system properties.


==> 4_model.tex <==


\section{HyperDynamics}
\label{sec:model}
The architecture of HyperDynamics  is illustrated in Figure \ref{fig:overview}. 
Given the agent and its environment, the agent first observes the environment and  interacts with it with a few actions. %, and records how the environments behaves. 
Then, a visual encoder $\Evisual$ encodes the visual observations into a latent visual feature code $\zvisual$, and our interaction encoder $\Einter$ encodes the interaction trajectory $\tau=(s_0,a_0,...s_{T},a_T)$  into a latent physics feature code $\zinter$. We consider a series of locomotion tasks for which only the interaction input is used, in accordance to precious works \cite{}, and a diverse object pushing task, in which the visual encoder encodes the 3D shape of the object, and is described in Section \ref{sec:encoder}. 
%These observations are then encoded into a latent feature code.
A \textit{hypernetwork} $\Eweight$ 
maps the concatenated code $z=[\zinter,\zvisual]$ to a set of neural network weights for the forward dynamics model $\ff$. 
%encoded codes and generates parameters of a \textit{target} forward dynamics model. 
The generated dynamics model $\ff$ learns a deterministic mapping from the state of the agent and the environment, and the action of the agent, to the  state change at the subsequent time step $t+1$; $\delta \xx_t = \ff^o(\xx_t, \act_t)$. 
For our locomotion tasks, the state contains only the state of the agent. For the object pushing task, the state is a concatenation of the 3D object location and the state of the agent $\xx_t=[\xx_t^{o},\xx_t^r]$. 


We train HyperDynamics by backpropagating error gradients of the prediction of the generated dynamics model, all the way to our visual and interaction encoders and the hypernetwork, the loss reads:  
%Let $\mathcal{O}$ denote the training object pool available. Let $T$ denote the length of a pushing trajectory. Let $N$ denote the number of trajectories per object. 
The  loss for our model for an input trajectory $\tau$ and input visual sensory input $I$ reads:
\begin{equation}
    %\mathcal{L}=  \frac{1}{ T } \sum_{t=1}^T \|\xx_{t+1} - \ff(\xx_t,\act_t;\Eweight(\zvisual ,\zinter)) \|_2
      \mathcal{L}=  \frac{1}{ T } \sum_{t=1}^T \|(\xx_{t+1}-\xx_t) - \ff(\xx_t,\act_t;\Eweight([\Evisual(I;\phi) ,\Einter(\tau;\psi))];\omega) \|_2
\end{equation}





%The 3D location of 

% \begin{figure*}[t]
% 	\centering
% 		\centering
% 		\includegraphics[width=\textwidth]{figures/arch.png}
% % 		\caption{Overview of HyperDynamics for object pushing. Given an object $o$, the shape encoder $\Eshape$ encodes the object's shape into $z_{shape}^o$, and the physics encoder $\Einter$ encodes the object's motion trajectory under a few random pushes into $z_{physics}^o$. These two vectors are fed into a hypernetwork $\Eweight$ to generate parameters to construct a dynamics model dedicated to $o$.\vspace{-20pt}}
% 		\caption{HyperDynamics for diverse object pushing. The shape encoder and the physics encoder together produce a latent code $z^o$ encoding object features, based on which a hypernetwork generates parameters of an expert dynamics model. }
% 			\label{fig:arch}
% \end{figure*}



\subsection{Encoding visual context for pushing objects}
%\label{sec:hypernet}

%Our framework takes as input the information regarding the shape and the physics properties of the object to predict neural weights that parameterize a corresponding expert dynamics model for that object.  
%The way objects move under pushing depends both on their shapes and physics properties, such as  mass, friction, restitution, etc. While the 3D object shape can be inferred by visual observation,  the physics properties  are hard to discern visually.  Instead, they can be inferred by observing the  motion of an object as a result to few (random) pokes from the robot \cite{xu2019densephysnet}.
Our model takes as input a 3D binary voxel occupancy grid representing the shape of the object and its motion trajectory under a few pokes, and predicts the parameters of a corresponding expert dynamic model, as shown in Figure \ref{fig:arch}.  


Let $V^o \in \{0,1\}^{w \times h \times d}$ denote an object-centric binary  occupancy voxel grid. We will consider $V^o$ to be provided by an oracle for now. A \textit{shape encoder} $\Eshape$ maps  $V^o$ to a 1-dimensional feature code $z^o_{shape} \in \mathbb{R}^{8}$.

\textbf{Object 3D orientation: context or state?} The shape of rigid objects does not change over time; rather, its orientation changes. The framework discussed so far intuitively divides the input information among different modules: the hypernetwork generates a dynamics model conditioned on system properties, and the dynamics model takes care of low-dimensional object state. However, when there's only a few objects used for training, the hypernetwork  will only strive to optimize for a discrete set of dynamics models, thus potentially leading to severe overfiting on the training data. Instead of feeding voxel grids of the objects with canonical poses to the shape encoder, we propose to use voxel grids oriented at the object's current orientation, and discard the orientation information in states fed into the generated dynamics model, as their weights already encode this information. Using oriented as opposed to canonical shape as input permits the hypernetwork $\hn$ to have way more training examples, even from a small number of objects with distinct shapes. 
Intuitively, $\hn$ now  treats the same object with different orientations as different objects, and generates a different expert for each. This helps smoothen and widen the data distribution seen by both the shape encoder and the hypernetwork, making the learning process much more sample-efficient. In addition, this also reduces burden for the  generated expert, by removing its need for processing orientation information.




%\subsection{Inferring Object Shape from 2.5D Images}
%\label{sec:single}
So far  we assumed access to ground-truth 3D occupancy voxel grids to represent the 3D shape of an object. Such information is readily available  in simulation  but unavailable in the real-world. 
We learn to map single view depth maps (2.5D) to  complete  3D feature grids $\M \in \mathbb{R}^{w \times h \times d \times c}$ that represent the appearance and shape of the scene and its objects by training Geometry-Aware Recurrent Networks (GRNN) of \cite{commonsense}. GRNNs learn to map RGB-D (2.5D) images to complete 3D feature grids of the scene they depict using differentiable unprojection (2.5D to 3D) and projection (3D to 2.5D) neural modules and 
can be optimized end-to-end to complete missing or occluded shape information, which is very useful for our tasks. We refer readers to \cite{commonsense} for more details. We apply GRNNs using only depth maps as input and disregard RGB information, since texture is less relevant to object pushing dynamics. We assume known object positions in our experiments, which in practice can be provided by a jointly trained 3D detection module with satisfactory accuracy \cite{commonsense}. We crop the scene map around the object to produce an object-centric map  $\M^o=\mathjrm{crop}(\M)$, which we use as the input for shape encoding. Though it is not the main contribution of this work, since we construct object-centric representations, our method is view-invariant; i.e., it does not require input images to be taken from a fixed viewpoint.

We also add additional regularization losses by autoencoding the object's shape, passing the shape code  $z^o_{shape}$ to a convolutional decoder $D_{shape}$ and minimizing a reconstruction loss. Note that the autoencoding loss can be applied to any object we have available, even objects not pushed by our agent, since acquiring massive shape data is cheap, as opposed to expensive simulation of actual pushing. In addition, since our tasks consider planar pushing, we found reconstructing a top-down 2D shape instead of the object's full 3D shape serves as a sufficient regularization task.

$ \underbrace{\|V^{o}_t- \Dshape(\Eshape(V^{o}_t)) \|_2}_{\text{shape autoencoding}}$

\subsection{Model Unrolling and Model Predictive Control}
\label{sec:MPC}
Action-conditioned dynamics model can be unrolled forward in time for long-term planning and subsequent control tasks.  The unrolling mechanism of HyperDynamics for pushing is straightforward: at each timestep $t$, a generated dynamics model $\ff^o_{t}$ predicts $\delta \xx_t^o$ for object $o$. Afterwards, we compute $\xx_{t+1}^o = \xx_t^o \oplus \delta \xx_t^o$, where $\oplus$ represents simple summation for positions and velocities, and quaternion composition for orientations. We then re-orient the 3D object-centric feature map $\M^o$ using the updated orientation $\mathbf{q}_{t+1}^o$ and generate a new dynamics model $\ff_{t+1}^o$. Finally, the updated full state $\xx_{t+1}^o$, excluding $\mathbf{q}_{t+1}^o$, is used by the updated dynamics model $\ff_{t+1}^o$ for motion prediction. 
We apply our approach with model predictive control (MPC) for pushing objects to desired target locations in scenes both with and without obstacles. When obstacles are at present, long-term planning is needed to generate collision-free action sequences. We unroll our model with randomly sampled action sequences, and evaluate each action sequence based on the Euclidean distance of the predicted end-location of the object from the target locations. We execute the first action of the best found action sequence and repeat the  process for a fixed time horizon $T$.




\paragraph{Implementation details}
The object state $\xx_t^{o}$ is a 13-vector containing the object's position $\mathbf{p}_t^o$ , orientation $\mathbf{q}_t^o$ (represented in quaternion), as well as its translational and rotational  velocities $\mathbf{v}_t^o$. The robot state $\delta \xx_t^{r}$ is a 3-vector representing the position of its end-effector. 
For controlling the robot, we use position-control in our experiments, so the action $\act_t = (\delta x, \delta y, \delta z)$ is a 3-vector representing the movement of the  robot's end-effector. Note that a PID controller controls the robot's torque in its joint  space under the hood, based on the  position-control commands, so varying the magnitude of the action could lead to different pushing speed of the end-effector. 
Given a pool of $N$ (training) objects and one robotic agent manipulating them, we will have a separate expert $\ff^o$ for modelling dynamics of each object $o$. 

We use fully-connected networks for $\Einter$  and $\Eweight$, and use a 3D convolutional network for $\Eshape$ without any heavy architecture search.

The hypernetwork generates all parameters in a single-shot as the output of it's final layer.

==> 4_model_xian_final_old.tex <==
\section{HyperDynamics for Object Pushing}
\label{sec:model}

Given a dynamical system with a certain set of properties, HyperDynamics first observes its  visual appearance, and then interacts with the system with a few actions and records how it behaves.
These observations are then encoded into a latent feature code.
A \textit{hypernetwork} takes as input this code and generates parameters of a \textit{target} forward dynamics model.
For our object pushing setting, we consider a robotic agent equipped with an RGB-D camera to observe the world and an end-effector to interact with it.
The agent's goal is to push objects to desired locations on a table surface.
Objects can vary in their physical properties, such as shape, mass, and friction relative to the table surface.

The architecture of HyperDynamics for pushing is illustrated in Figure \ref{fig:arch}. It consists of three main modules: an object feature encoder (comprised of a \textit{shape encoder} and a \textit{physics encoder}), a  \textit{hypernetwork} for neural weights generation, and a \textit{dynamics model} for motion prediction. The dynamics model is a forward temporal predictive model that takes as input a low-dimensional representation of the state of the object and the agent, as well as the action of the agent at time step $t$, and predicts the next state for the object and the agent. The state of the object  purposefully does not include information regarding the visual appearance or physics properties of the object, since these properties do not change over time. We thus use the term \textit{expert} to refer to a dynamics model for a specific object.   Such expert dynamics models are popular formulations in the literature. As a matter of fact, it's been shown recently that modelling epistemic and aleatoric uncertainty of such expert models during unrolling permits  model-based formulation to surpass  model-free RL (in manipulating a single object or controlling a single system) both in low- and high-data regimes \cite{NIPS2018_7725}. Our framework  generalizes such formulation by predicting their parameters using a hypernetwork that conditions on visual appearance and physics properties of the object in hand. The only difference is that instead of directly optimizing the weights of such expert dynamics models \cite{NIPS2018_7725}, we will be predicting them using a hypernetwork. Our model is trained by back-propagating the expert model's prediction error in an end-to-end differentiable manner.

\begin{figure*}[t]
	\centering
		\centering
		\includegraphics[width=\textwidth]{figures/arch.png}
% 		\caption{Overview of HyperDynamics for object pushing. Given an object $o$, the shape encoder $\Eshape$ encodes the object's shape into $z_{shape}^o$, and the physics encoder $\Einter$ encodes the object's motion trajectory under a few random pushes into $z_{physics}^o$. These two vectors are fed into a hypernetwork $\Eweight$ to generate parameters to construct a dynamics model dedicated to $o$.\vspace{-20pt}}
		\caption{Overview of HyperDynamics for object pushing. The shape encoder and the physics encoder together produce a latent code $z^o$ encoding object features, based on which a hypernetwork generates parameters of an expert dynamics model. \vspace{-18pt}}
			\label{fig:arch}
\end{figure*}

We describe our expert dynamics models in Section \ref{sec:expert} and how we generate them  in Section \ref{sec:hypernet}. 
We discuss using HyperDynamics for temporal unrolling and model predictive control in Section \ref{sec:MPC}. In order to obtain the shape property, we will first assume access to ground-truth 3D voxel  grids of the objects, and then discuss in Section \ref{sec:single} how we relax this assumption and infer object shapes using 2.5D single-view images. Note that a vast majority of prior works in modelling object dynamics  consider only quasi-static pushing or poking, in which an object always starts to move or  stops together with the robot's end-effector \cite{DBLP:journals/corr/FinnL16, agrawal2016learning, li2018push, pinto2017learning}. We go beyond simple quasi-static pushing by varying the physics parameters of the object and the scene, and allow an object to slide by itself if pushed with a high speed. 



\subsection{Expert Dynamics Models}
\label{sec:expert}

The expert dynamics model $\ff^o$ learns a deterministic mapping from the state of an object $\xx_t^{o}$, the state of the robot's end-effector $\xx_t^{r}$, and an action applied by the agent $\act_t$  at timestep $t$, to  the  state change at the subsequent time step $t+1$; i.e. $\delta \xx_t = \ff^o(\xx_t, \act_t)$,  where $\delta \xx_t = <\delta \xx_t^{o}, \delta \xx_t^{r}>$ includes state change for both the object and the robot.   
The object state $\xx_t^{o}$ is a 13-vector containing the object's position $\mathbf{p}_t^o$ , orientation $\mathbf{q}_t^o$ (represented in quaternion), as well as its translational and rotational  velocities $\mathbf{v}_t^o$. The robot state $\delta \xx_t^{r}$ is a 3-vector representing the position of its end-effector.

For controlling the robot, we use position-control in our experiments, so the action $\act_t = (\delta x, \delta y, \delta z)$ is a 3-vector representing the movement of the  robot's end-effector. Note that a PID controller controls the robot's torque in its joint  space under the hood, based on the  position-control commands, so varying the magnitude of the action could lead to different pushing speed of the end-effector. 
Given a pool of $N$ (training) objects and one robotic agent manipulating them, we will have a separate expert $\ff^o$ for modelling dynamics of each object $o$. 

%In our setting, $\xx_t^{o}$ is a 13-vector containing the object's position $p_t^{o} \in \mathbb{R}^3$, orientation $q_t^{o} \in \mathbb{R}^3$ (represented as quaternion), as well as its translational and rotational velocities $v_t^{o} \in \mathbb{R}^6$. \todo{how it is 13?} %We have $\xx_{t+1}= \xx_t+ \delta \xx_t$. 
%$\delta x_t^{obj}$ is a vector with the same size representing the change in the object's position, orientation and velocity. The same applies to $x_t^{rob}$  and $\delta x_t^{rob}$. 


%We  train a ensemble of $N$ experts, one for each object,  and use them as a reference for experimental comparison.
%\subsection{Encoding Object Features}
%\label{sec:encoder}

\subsection{Generating Neural Weights for Expert Dynamics Models }
\label{sec:hypernet}

Our framework takes as input the information regarding the shape and the physics properties of the object to predict neural weights that parameterize a corresponding expert dynamics model for that object.  
The way objects move under pushing depends both on their shapes and physics properties, such as  mass, friction, restitution, etc. While the 3D object shape can be inferred by visual observation,  the physics properties  are hard to discern visually.  Instead, they can be inferred by observing the  motion of an object as a result to few (random) pokes from the robot \cite{xu2019densephysnet}.
Our model takes as input a 3D binary voxel occupancy grid representing the shape of the object and its motion trajectory under a few pokes, and predicts the parameters of a corresponding expert dynamic model, as shown in Figure \ref{fig:arch}.  


Let $V^o \in \{0,1\}^{w \times h \times d}$ denote an object-centric binary  occupancy voxel grid. We will consider $V^o$ to be provided by an oracle for now. A \textit{shape encoder} $\Eshape$ maps  $V^o$ to a 1-dimensional feature code $z^o_{shape} \in \mathbb{R}^{8}$.
Let $\tau^o \in \mathbb{R}^{3 \times T_{inter}}$ denote the trajectory of object displacements when pushed for $T_{inter}$ timesteps, where the pushing actions are from random directions but with same  magnitudes. We found  $T_{inter}=5 $  sufficient  to yield good performance and used it in  all our experiments. 
A \textit{physics encoder} $\Einter$ maps the trajectory to a 1-dimensional code $z_{physics}^o \in \mathbb{R}^{2}$ that represents information regarding the physical properties of the object. 
A \textit{hypernetwork} $\Eweight$ maps the concatenated code $z^o=[z^o_{shape},z^o_{physics}]$ to a set of neural network weights for the dynamics expert $\ff$  described in Section \ref{sec:expert}. The hypernetwork generates all parameters in a single-shot as the output of it's final layer. To better evaluate our framework, we aim for simplicity of each network modules. We use fully-connected networks for $\Einter$  and $\Eweight$, and use a 3D convolutional network for $\Eshape$ without any heavy architecture search.

We train HyperDynamics by backpropagating error gradients of the prediction of the generated dynamics model, all the way to our shape and physics encoders and the hypernetwork.  
We also add additional regularization losses by autoencoding the object's shape, passing the shape code  $z^o_{shape}$ to a convolutional decoder $D_{shape}$ and minimizing a reconstruction loss. 
Let $\mathcal{O}$ denote the training object pool available. Let $T$ denote the length of a pushing trajectory. Let $N$ denote the number of trajectories per object. 
The final loss for our model reads:
\begin{equation}
    \mathcal{L}=  \frac{1}{|\mathcal{O}| T } \sum_{t=1}^T \sum_{o=1}^{|\mathcal{O}|}\underbrace{\|\xx^o_{t+1} - \ff(\xx^o_t,\act^o_t;\Eweight(z^{o,t}_{shape},z^o_{physics})) \|_2}_{\text{dynamics prediction}} + \underbrace{\|V^{o}_t- \Dshape(\Eshape(V^{o}_t)) \|_2}_{\text{shape autoencoding}}
\end{equation}

Note that the autoencoding loss can be applied to any object we have available, even objects not pushed by our agent, since acquiring massive shape data is cheap, as opposed to expensive simulation of actual pushing. In addition, since our tasks consider planar pushing, we found reconstructing a top-down 2D shape instead of the object's full 3D shape serves as a sufficient regularization task.

\textbf{Object 3D orientation: context or state?} The shape of rigid objects does not change over time; rather, its orientation changes. The framework discussed so far intuitively divides the input information among different modules: the hypernetwork generates a dynamics model conditioned on system properties, and the dynamics model takes care of low-dimensional object state. However, when there's only a few objects used for training, the hypernetwork  will only strive to optimize for a discrete set of dynamics models, thus potentially leading to severe overfiting on the training data. Instead of feeding voxel grids of the objects with canonical poses to the shape encoder, we propose to use voxel grids oriented at the object's current orientation, and discard the orientation information in states fed into the generated dynamics model, as their weights already encode this information. Using oriented as opposed to canonical shape as input permits the hypernetwork $\hn$ to have way more training examples, even from a small number of objects with distinct shapes. 
Intuitively, $\hn$ now  treats the same object with different orientations as different objects, and generates a different expert for each. This helps smoothen and widen the data distribution seen by both the shape encoder and the hypernetwork, making the learning process much more sample-efficient. In addition, this also reduces burden for the  generated expert, by removing its need for processing orientation information.




\subsection{Inferring Object Shape from 2.5D Images}
\label{sec:single}
So far  we assumed access to ground-truth 3D occupancy voxel grids to represent the 3D shape of an object. Such information is readily available  in simulation  but unavailable in the real-world. 
We learn to map single view depth maps (2.5D) to  complete  3D feature grids $\M \in \mathbb{R}^{w \times h \times d \times c}$ that represent the appearance and shape of the scene and its objects by training Geometry-Aware Recurrent Networks (GRNN) of \cite{commonsense}. GRNNs learn to map RGB-D (2.5D) images to complete 3D feature grids of the scene they depict using differentiable unprojection (2.5D to 3D) and projection (3D to 2.5D) neural modules and 
can be optimized end-to-end to complete missing or occluded shape information, which is very useful for our tasks. We refer readers to \cite{commonsense} for more details. We apply GRNNs using only depth maps as input and disregard RGB information, since texture is less relevant to object pushing dynamics. We assume known object positions in our experiments, which in practice can be provided by a jointly trained 3D detection module with satisfactory accuracy \cite{commonsense}. We crop the scene map around the object to produce an object-centric map  $\M^o=\mathjrm{crop}(\M)$, which we use as the input for shape encoding. Though it is not the main contribution of this work, since we construct object-centric representations, our method is view-invariant; i.e., it does not require input images to be taken from a fixed viewpoint.


\subsection{Model Unrolling and Model Predictive Control}
\label{sec:MPC}
Action-conditioned dynamics model can be unrolled forward in time for long-term planning and subsequent control tasks.  The unrolling mechanism of HyperDynamics for pushing is straightforward: at each timestep $t$, a generated dynamics model $\ff^o_{t}$ predicts $\delta \xx_t^o$ for object $o$. Afterwards, we compute $\xx_{t+1}^o = \xx_t^o \oplus \delta \xx_t^o$, where $\oplus$ represents simple summation for positions and velocities, and quaternion composition for orientations. We then re-orient the 3D object-centric feature map $\M^o$ using the updated orientation $\mathbf{q}_{t+1}^o$ and generate a new dynamics model $\ff_{t+1}^o$. Finally, the updated full state $\xx_{t+1}^o$, excluding $\mathbf{q}_{t+1}^o$, is used by the updated dynamics model $\ff_{t+1}^o$ for motion prediction. 
We apply our approach with model predictive control (MPC) for pushing objects to desired target locations in scenes both with and without obstacles. When obstacles are at present, long-term planning is needed to generate collision-free action sequences. We unroll our model with randomly sampled action sequences, and evaluate each action sequence based on the Euclidean distance of the predicted end-location of the object from the target locations. We execute the first action of the best found action sequence and repeat the  process for a fixed time horizon $T$.


==> 5_experiments.tex <==
\section{Experiments}\label{sec:experiments}

Most prior works that learn object dynamics  consider only quasi-static pushing or poking, in which an object always starts to move or  stops together with the robot's end-effector \cite{DBLP:journals/corr/FinnL16, agrawal2016learning, li2018push, pinto2017learning}. We go beyond simple quasi-static pushing by varying the physics parameters of the object and the scene, and allow an object to slide by itself if pushed with a high speed. 



We test our proposed method on its motion prediction accuracy for single- and multi-step pushing, as well as its performance when used for pushing objects to desired locations with MPC. We train our model with data generated using the PyBullet simulator \cite{coumans2019}. Our setup uses a Kuka robotic arm equipped with a single rod-shaped end-effector, as shown in Figure \ref{fig:arch}. Our dataset consists of only 31 different object meshes with distinct shapes, including 11 objects from the MIT Push dataset \cite{mitpush} and 20 objects selected from four categories (\textit{camera}, \textit{mug}, \textit{bowl} and \textit{bed}) in the ShapeNet Dataset \cite{shapenet2015}. We split our dataset so that 24 objects are used for training and 7 are used for testing. The objects can move freely on a planar table surface of size $0.6m\times0.6m$. For data collection, we randomly sample one object with randomized mass and friction coefficient, and place it on the table with a random starting position. Then, we instantiate the end-effector nearby the object and collect pushing sequences with length of 5 timesteps, where each action is a random horizontal displacement of the robot's end-effector  ranging from $3cm$ to $6cm$, and each timestep is defined to be $800ms$. Our method is view-invariant and relies on a single 2.5D image as input. When collecting data, we place cameras at 9 different views around the table. At test time, we use a single and randomly selected view. Note that although collecting actual interactions with objects is expensive and time-consuming, data consisting of only varying shapes are cheap and easily accessible. To ensure $z_{shape}^o$ produced by the shape encoder $\Eshape$ captures sufficient shape information for pushing, we train it on the whole ShapeNet \cite{shapenet2015} for shape autoencoding as an auxiliary task, jointly with the dynamics prediction task. 

Our experiments aim to evaluate the performance of the automatically generated expert models, as well as to compare our model with alternative formulations which optimizes a single global dynamics model, as commonly shown in the current literature. We compare our model against the following baselines:
\begin{itemize}
    \item \textit{XYZ}: a model that only take as input the action and states of the object and the agent, without having access to its visual feature or physics properties, similar to \cite{DBLP:journals/corr/abs-1808-00177, wu2017learning}.
    
    \item \textit{Direct}: this model uses the same input information as our model does. The only difference is that it directly optimizes a single global dynamics model instead of generating experts. This approach resembles the most common way of conditioning on object features  used in the current literature \cite{DBLP:journals/corr/FinnL16, agrawal2016learning, li2018push, densephysnet, Fragkiadaki2015LearningVP, zhang2019solar, hafner2019planet}, where a global dynamics model takes as input both the state and properties of the dynamical system.
    \item Visual Foresight (\textit{VF})\cite{DBLP:journals/corr/FinnL16} and \textit{DensePhysNet}\cite{densephysnet}: these two models rely on 2D visual inputs of the current frame, and predict 2D optical flows that transform the current frame to the future frame. These models also use a global dynamics model for varying system properties, and feed system features directly into the model, following the same philosophy of \textit{Direct}. Compared to \textit{VF}, \textit{DensePhysNet} uses a multi-step aggregator to infer physics properties from a history of previous interactions, and it also uses a cross-convolution layer 
   to couple system features and action signals more effectively \cite{xue2016visual}.
   \item \textit{Expert-Ens}: we train a separate expert model for each distinct object, forming an ensemble of experts. These experts assume access to \textit{ground-truth} orientation, mass, and friction information. The performance of this baseline when tested on objects seen during training represents the theoretically optimal performance, and our model aims to match it. For novel objects, we retrieve the nearest-neighbour object in terms of shape in the training set, and use its corresponding expert for evaluation.
   
\end{itemize}

In Appendix, we include details of our experimental setup (Section A) and the baselines (Section B). We also show a comparison with dynamics models meta-trained with MAML \cite{clavera} (Section C.1), and additional qualitative results of how our model transfers to real-world scenarios (Section C.2).

\input{tables}

% \begin{table}[t]
% 	\begin{minipage}{0.5\linewidth}
% 		\caption{Motion Prediction Error}
% 		\label{table:motion}
% 		\centering
% 		\begin{tabular}{lcccc}
%     \toprule
%                                       & \multicolumn{2}{c}{Seen objects} & \multicolumn{2}{c}{Novel objects} \\
%                                       & $t=1$             & $t=5  $          & $t=1 $            & $t=5  $           \\
%          \midrule
% Expert-Ens  &   \textbf{\textit{0.70}}            &     \textbf{\textit{3.98}}          &         1.44        &        5.50         \\ 
%       \midrule      
% Ours      &     \textbf{0.70}             &            \textbf{4.04}       &        \textbf{0.85}          &      \textbf{4.53}           \\
%     \cmidrule(r){1-5}
% Direct   &      0.83           &      4.62          &     1.03            &           5.28    \\
%     \cmidrule(r){1-5}
% XYZ     &       1.28          &        5.35        &        1.51         &          6.00       \\ 
%     \bottomrule 
% \end{tabular}
% 	\end{minipage}\hfill
% 	\begin{minipage}{0.45\linewidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{figures/comp.png}
% 		\captionof{figure}{Comparison of Prediction Error}
% 		\label{fig:comp}
% 	\end{minipage}
% 	\vspace{-15pt}
% \end{table}

\subsection{Single- and Multi-step Motion Prediction}

We evaluate performance of our model on prediction error in Table \ref{table:motion} for both single-step ($t=1$) and multi-step unrolling ($t=5$). Red numbers in bold denote the best performance across all models, while black numbers in bold represent the theoretically optimal performance (provided by the \textit{Expert-Ens}). For multi-step unrolling, we condition on the first frame of a sampled trajectory, and roll out the model forward in a recurrent way. Note that \textit{VF} and \textit{DensePhysNet} are not included here since they work in 2D image space and do not predict explicit object motion. When tested on objects seen during training, while our model needs to infer orientation information and physics properties via encoding visual input and interactions, it performs on par with the optimal \textit{Expert-Ens}, which assumes access to ground-truth orientation, mass and friction coefficient. This shows that the dynamics model generated by HyperDynamics on the fly is as performant as the separately and directly trained dynamics experts.  We also show the error comparison for single-step prediction in Figure \ref{fig:comp}, to better visualize the performance difference across all models. The \textit{XYZ} baseline depicts the best performance possible when  shape and physics properties of the objects are unknown. When tested with novel objects unseen during training, our model shows a performance similar to seen objects, outperforming \textit{XYZ} by a great margin, demonstrating that our model transfers acquired knowledge to novel objects well. \textit{Expert-Ens} on novel objects performs as bad as \textit{XYZ}, suggesting that with only a handful of distinct objects in the training set, applying these dedicated models to novel objects, though after nearest-neighbour search, yields unsatisfactory performance. The \textit{Direct} baseline  shows acceptable performance for both seen and novel objects, but is at a clear disadvantage when compared to ours. This suggests that in the context of object pushing,  our hierarchical way of conditioning on system features and generating experts outperforms the common framework which uses a global model with fixed parameters for varying system dynamics.



\subsection{Pushing with Model Predictive Control (MPC)}
We test the performance of our model for downstream manipulation tasks, where the robot needs to push the objects to desired target locations. We consider pushing both with and without obstacles. We place a randomly selected object in the scene with a random initial position, and sample a random target location for it. At each step, we evaluate 30 random action sequences with the model before taking an action. For pushing without obstacle, the maximum distance of the target to the initial position for each object is capped at $0.25m$, and a planning horizon of 1 step is used since greedy action selection suffices for it. For pushing with obstacles, we randomly place 2 additional obstacles in the scene, selected from the same pool of available objects. The distance from the target to the initial position is uniformly sampled from the range $[0.24m, 0.40m]$. The model needs to plan a collision free path and thus a planning horizon of 10 steps is used.

For both tasks, we run 50 trials and evaluate the success rate, where it is considered successful if the object ends up within $4cm$ from the target position, without colliding with any obstacles along the way. \textit{VF} and \textit{DensePhysNet} does not predict explicit object state so they are not applicable for collision-checking during unrolling, thus we only compare with them for pushing without obstacles.
Results of all the models are shown in Table \ref{tab:mpc}. Again, our models shows similar performance as the \textit{Expert-Ens} when evaluated on seen objects, and outperforms it by a margin on novel objects. Note that since \textit{DensePhysNet} takes into accuont the history of interactions, it is able to infer physicis properties and outperforms \textit{VF}, which is designed to consider only quasi-static pushing. Our model shows a better performance when used for planning and control compared with all the baseline models. 

% \begin{table}[]
%   \caption{Success Rate for Object Pushing with MPC}
%   \label{tab:mpc}
% \begin{tabular}{@{}llcccccc@{}}
%     \toprule
%                               & 
%                               & Expert-Ens & Ours & Direct & XYZ & VF & DensePhysNet \\
%                               \midrule
% \multirow{2}{*}{w/o obstacles}  & seen objects   &   \textbf{\textit{0.94}}&  \textbf{0.94}    &     0.92   & 0.84    & 0.62   &        0.70      \\
% \cmidrule(r){2-8}
%                               & novel objects &    0.80        &   \textbf{0.94}   &   0.88      &  0.76 &  0.52  &  0.58            \\
%                               \midrule
% \multirow{2}{*}{w/ obstacles} & seen objects   &      \textbf{\textit{0.72}}      &   \textbf{0.70}   &  0.66      &   0.48  & --- & ---         \\
% \cmidrule(r){2-8}
%                               & novel objects  &  0.48          & \textbf{0.68}     &   0.62     &   0.46  &  --- & ---   \\
% \bottomrule
% \end{tabular}\vspace{-10pt}
% \end{table}

\paragraph{Limitations}
Our model currently has three main limitations. \textbf{(i)} When multiple objects are in the scene, our structured object-centric representation does allow the robot to interact with each of them separately and is able to predict future states. However, since we treat object properties as contextual information to model robot-object interactions, our framework currently does not support modeling for cross-object interactions. Combining our framework with Graph Neural Networks \cite{battaglia2016interaction} and encode features of all objects together in an unordered manner to model cross-object interactions would be an interesting extension in the future. \textbf{(ii)} Our model learns dynamics of rigid objects. Modeling dynamics of soft bodies or fluids requires predicting a 3D dense flow field. We will investigate this with simulators supporting soft bodies and fluids \cite{DBLP:journals/corr/abs-1810-05762} in the future. 
\textbf{(iii)} Our model is deterministic. Adding stochasticity to our framework by combining it with stochastic neural networks \cite{kingma2013auto,liu2016stein}  for predicting object motions with multi-modalities is our future work.




==> 6_conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
We presented HyperDynamics,  as model that  learns dynamics by generating low-dimensional dynamics functions from interactions and visual context of the scene and the agent. We compared HyperDynamics with representative models in the literature and showed superior generalization of the dynamics learnt on locomotion at test novel conditions and on pushing novel objects.


Our model currently has three main limitations. \textbf{(i)} When multiple objects are in the scene, our structured object-centric representation does allow the robot to interact with each of them separately and is able to predict future states. However, since we treat object properties as contextual information to model robot-object interactions, our framework currently does not support modeling for cross-object interactions. Combining our framework with Graph Neural Networks \cite{battaglia2016interaction} and encode features of all objects together in an unordered manner to model cross-object interactions would be an interesting extension in the future. \textbf{(ii)} Our model learns dynamics of rigid objects. Modeling dynamics of soft bodies or fluids requires predicting a 3D dense flow field. We will investigate this with simulators supporting soft bodies and fluids \cite{DBLP:journals/corr/abs-1810-05762} in the future. 
\textbf{(iii)} Our model is deterministic. Adding stochasticity to our framework by combining it with stochastic neural networks \cite{kingma2013auto,liu2016stein}  for predicting object motions with multi-modalities is our future work.



Handling more varied visual tasks and predicting both the structure and the parameters of the target dynamics model are interesting avenues for future work. We hope the current work  to stimulate research into weight generation for adaptation of models and dynamics in versatile ++
%the dynamics learning research community. % into inves

%and leave evaluations of the proposed architecture for other dynamics tasks as future work.

%in the context of object pushing. Our approach observes the object's visual apperances and its behavior under a handful of interactions, and generate an expert dynamics model dedicated to the observed object on the fly. 
%Our experiments show that HyperDynamics for pushing is sufficient to generate  expert models that perform on par with the directly trained ensemble of experts, while other baseline approaches fail to do so. In addition, with only 24 objects in our training set, HyperDynamics is able to transfer learned knowledge to novel objects effectively, showing only a small performance gap when tested on seen and novel objects. 

%We believe the performance gain is acquired from the hierarchical way of processing and decoupling input signals: we condition on system property information, and generate parameters that constructs a dedicated dynamics model to process the
% state information in a multiplicative way.
 
%Note that HyperDynamcis is a general framework that is \textit{potentially} applicable to a wide range of dynamics learning tasks. For example, we  could generate controllers for legged robots  conditioned  on their morphology; we can observe how a robotic manipulator moves based on  given control commands, and generate an updated dynamics model for it in case of any changes in system behavior due to motor  replacement or gear wearing; we can also condition on  trajectories  of a robotic swimmer, and infer physical properties of the system (such as friction and viscosity of the water), and adapt the dynamics model used for control. We hope this work of using HyperDynamics for modeling interactions with objects could inspire the dynamics learning research community, and leave evaluations of the proposed architecture for other dynamics tasks as future work.



%Extending this model to non-rigid object dynamics, 
% \todo{self-supervision} and stochastic transitions are  clear avenues for future work. 


%\paragraph{Acknowledgements} This work was partially funded by Sony AI. 


==> 6_conclusion_xian_final.tex <==
\section{Conclusion} \label{sec:conclusion}
We presented HyperDynamics as a framework for learning dynamics in the context of object pushing. Our approach observes the object's visual apperances and its behavior under a handful of interactions, and generate an expert dynamics model dedicated to the observed object on the fly. Our experiments show that HyperDynamics for pushing is sufficient to generate  expert models that perform on par with the directly trained ensemble of experts, while other baseline approaches fail to do so. In addition, with only 24 objects in our training set, HyperDynamics is able to transfer learned knowledge to novel objects effectively, showing only a small performance gap when tested on seen and novel objects. We believe the performance gain is acquired from the hierarchical way of processing and decoupling input signals: we condition on system property information, and generate parameters that constructs a dedicated dynamics model to process the
 state information in a multiplicative way.
 
Note that HyperDynamcis is a general framework that is \textit{potentially} applicable to a wide range of dynamics learning tasks. For example, we  could generate controllers for legged robots  conditioned  on their morphology; we can observe how a robotic manipulator moves based on  given control commands, and generate an updated dynamics model for it in case of any changes in system behavior due to motor  replacement or gear wearing; we can also condition on  trajectories  of a robotic swimmer, and infer physical properties of the system (such as friction and viscosity of the water), and adapt the dynamics model used for control. We hope this work of using HyperDynamics for modeling interactions with objects could inspire the dynamics learning research community, and leave evaluations of the proposed architecture for other dynamics tasks as future work.



%Extending this model to non-rigid object dynamics, 
% \todo{self-supervision} and stochastic transitions are  clear avenues for future work. 


%\paragraph{Acknowledgements} This work was partially funded by Sony AI. 


==> Abstract.tex <==

\begin{abstract}
We propose HyperDynamics, a model that generates parameters of neural dynamics models for a particular environment by conditioning on an agent's  interactions with that environment and optionally its visual observations. 
The generated model  operates over the dynamics of instantaneous low-dimensional state representations of the agent and its environment. Physical and visual properties of the environment that are not part of the low-dimensional state yet affect its temporal  dynamics are inferred from the interaction history and visual observations, and are implicitly captured in the generated parameters.  
We test HyperDynamics  on a set of object pushing and locomotion tasks, where the objects to push and locomotion environments vary. 
HyperDynamics outperform existing dynamics models in the literature that adapt to  environment variations by  learning dynamics over high dimensional visual observations, capturing the interactions of the agent in  recurrent state representations,  or using gradient-based meta-optimization.
We  show that HyperDynamics matches the performance of an ensemble of separately trained dynamics experts in our training environments and generalizes well to unseen environment variations at test time.
We attribute its good performance over existing model adaptation methods to the multiplicative interactions between the inferred environment properties---captured in the generated parameters---and the low-dimensional state representation of the environment.

% Why are there two abstracts? Is this the one supposed to be the final one?

\end{abstract}



==> Exps.tex <==
\section{Experiments}\label{sec:experiments}
Our experiments aim to answer the following questions: (1) Is \HD \ able to generate dynamics models across environment variations that perform as well as expert dynamics models, trained specifically on the dynamics of each environment variation?  (2) Does \HD\  generalize to environments with novel properties ? 
(3) How does \HD \ compare with methods that either use fixed global dynamics models or adapt their parameters  during the course of interaction through meta-optimization?
We test our proposed framework in the contexts of both object pushing and locomotion, and describe each of them in details below.

\subsection{Object Pushing}
Many prior works that learn object dynamics consider only quasi-static pushing or poking, where an object always starts to move or  stops together with the robot's end-effector \citep{DBLP:journals/corr/FinnL16, agrawal2016learning, li2018push, pinto2017learning}. We go beyond simple quasi-static pushing by varying the physics parameters of the object and the scene, and allow an object to slide by itself if pushed with a high speed. A PID controller controls the robot's torque in its joint  space under the hood, based on position-control commands, so varying the magnitude of the action could lead to different pushing speed of the end-effector. 
We test \HD\ on its motion prediction accuracy for single- and multi-step object pushing, as well as its performance when used for pushing objects to desired locations with MPC.

\paragraph{Experimental Setup} We train our model with data generated using the PyBullet simulator \citep{coumans2019}. Our setup uses a Kuka robotic arm equipped with a single rod-shaped end-effector, as shown in Figure \ref{fig:overview}. Our dataset consists of only 31 different object meshes with distinct shapes, including 11 objects from the MIT Push dataset \citep{mitpush} and 20 objects selected from four categories (\textit{camera}, \textit{mug}, \textit{bowl} and \textit{bed}) in the ShapeNet Dataset \citep{shapenet2015}. We split our dataset so that 24 objects are used for training and 7 are used for testing. The objects can move freely on a planar table surface of size $0.6m\times0.6m$. For data collection, we randomly sample one object with randomized mass and friction coefficient, and place it on the table with a random starting position. Then, we instantiate the end-effector nearby the object and collect pushing sequences with length of 5 timesteps, where each action is a random horizontal displacement of the robot's end-effector  ranging from $3cm$ to $6cm$, and each timestep is defined to be $800ms$. Our method relies on a single 2.5D image as input for object detection and motion prediction. Note that although collecting actual interactions with objects is expensive and time-consuming, data consisting of only varying shapes are cheap and easily accessible. To ensure $z_{shape}^o$ produced by the shape encoder $\Eshape$ captures sufficient shape information for pushing, we train it on the whole ShapeNet \cite{shapenet2015} for \todo{shape perpective to top-down view prediction as an auxiliary task}, jointly with the dynamics prediction task. Please refer to Appendix \ref{sec:ap-exp} for more details of our experimental setup.


\paragraph{Baselines} We compare our model against these baselines: 
\textbf{(1)} \textit{XYZ}: a model that  takes as input the action and states of the object and the agent, without having access to its visual feature or physics properties, similar to \citet{DBLP:journals/corr/abs-1808-00177} and \citet{wu2017learning}. 
\textbf{(2)} \textit{Direct}: a model that uses the same $\Evisual$ and $\Einter$ as our model does. The only difference is that it directly optimizes a single global dynamics model instead of generating experts. This approach resembles the most common way of conditioning on object features  used in the current literature \citep{DBLP:journals/corr/FinnL16, agrawal2016learning, li2018push, densephysnet, Fragkiadaki2015LearningVP, zhang2019solar, hafner2019planet}, where a global dynamics model takes as input both the state and properties of the dynamical system. 
\textbf{(3)} Visual Foresight (\textit{VF}) \citep{ebert2018visual} and \textit{DensePhysNet} \citep{densephysnet}: these two models rely on 2D visual inputs of the current frame, and predict 2D optical flows that transform the current frame to the future frame. These models also use a global dynamics model for varying system properties, and feed system features directly into the model, following the same philosophy of \textit{Direct}. 
\textbf{(4)} \textit{MB-MAML} \citep{Nagabandi2019LearningTA}: a meta-trained model which applies model-agnostic meta-learning (MAML) to model-based RL, and trains a dynamics model prior that can be rapidly adapted to the local context when given newly observed data. \textbf{(5)} \textit{Expert-Ens}: we train a separate expert model for each distinct object, forming an ensemble of experts. These experts assume access to \textit{ground-truth} orientation, mass, and friction information. This baseline serves as an oracle when tested on seen objects during training. For unseen objects, we select a corresponding expert from the ensemble by shape-based nearest-neighbour retrieval, essentially performing explicit system identification.
\input{table_push}


We evaluate all the methods on prediction error for both single-step ($t=1$) and multi-step unrolling ($t=5$) (Table \ref{table:motion}). We also test their performance for downstream manipulation tasks, where the robot needs to push the objects to desired target locations with MPC, in scenes both with and without obstacles. When obstacles are at present, the agent needs to plan a collision-free path. We report their success rates in 50 trials in Table \ref{tab:mpc}. Red numbers in bold denote the best performance across all models, while black numbers in bold represent oracle performance (provided by \textit{Expert-Ens}). \textit{VF} and \textit{DensePhysNet} are not tested for motion prediction since they work in 2D image space and do not predict explicit object motion, and are not applicable for collision checking and collision-free pushing for the same reason. 

Our model outperforms all baselines by a margin on both prediction and control tasks. When tested on objects seen during training, while our model needs to infer orientation information and physics properties via encoding visual input and interactions, it performs on par with the \textit{Expert-Ens} oracle, which assumes access to ground-truth orientation, mass and friction coefficient. This shows that the dynamics model generated by HyperDynamics on the fly is as performant as the separately and directly trained dynamics experts. The \textit{XYZ} baseline depicts the best performance possible when  shape and physics properties of the objects are unknown. When tested with novel objects unseen during training, our model shows a performance similar to seen objects, outperforming \textit{XYZ} by a great margin, demonstrating that our model transfers acquired knowledge to novel objects well. \textit{Expert-Ens} on novel objects performs similarly to \textit{XYZ}, suggesting that with only a handful of distinct objects in the training set, applying these dedicated models to novel objects, though after nearest-neighbour searches, yields poor generalization. Performance gain of our model over \textit{Direct} suggests our hierarchical way of conditioning on system features and generating experts outperforms the common framework in the literature, which uses a global model with fixed parameters for varying system dynamics. Our model also shows a clear performance gain over \textit{MB-MAML}, when only 5 data samples of interaction are available for online adaptation. This indicates that our framework, which directly generates dynamics model given the system properties, is much more sample-efficient than the meta-trained dynamics model prior that needs to adapt to the context via extra tuning. 


\begin{wrapfigure}{tr}{0.45\textwidth}
\vspace{-8ex}
  \begin{center}
		\includegraphics[width=0.44\textwidth]{figures/locomotion.png}
		\caption{We consider two types of robots and two environments for locomotion. Top: Ant-Pier. Down: Cheetah-Slope.}
		\label{fig:loco}
  \end{center}
\vspace{-6ex}
\end{wrapfigure}
\subsection{Locomotion}

Below,  \HD\ works on more complex RL problems other than object pushing, we also study on several locomotion tasks.
\paragraph{Experimental Setup} We set up our environment using the MuJoCo simulator \citep{todorov2012mujoco}. In particular, we consider two types of robots: a planar cheetah and a quadrupedal ``ant'' robot. For each robot, we consider two environments where the terrains are changing: (1) \textit{Slope}: the robot needs to walk over a terrain consisting of multiple slopes with changing steepness. (2) \textit{Pier}: the robot needs to walk over a series of blocks floating on the water surface, where damping and friction properties vary between the blocks. As a result, we consider these 4 tasks in total: \textit{Cheetah-Slope}, \textit{Ant-Slope}, \textit{Cheetah-Pier} and \textit{Ant-Pier}. Figure \ref{fig:loco} shows two of them. Unlike the setting of object pushing, in the context of locomotion it's unrealistic to assume arbitrary resetting of robot states for data collection. As a result, on-policy data collection is performed: the latest model is used for action selection to collect best-performing trajectories, which are then used to update the dataset for model training. For \textit{Slope}, the environment is comprised of a series of consecutive terrain segments, each of which has a randomly sampled steepness. During test time, we also evaluate on unseen terrains with either higher of lower steepness. For \textit{Pier}, each of the blocks floating on the water has randomly sampled friction and damping properties, and moves vertically when the robot runs over it, resulting in a rapidly changing terrain. Similarly, during test time we also evaluate using blocks with properties outside of the training distribution. See Appendix \ref{sec:ap-exp} for more details.

\paragraph{Baselines} We compare our model against these baselines: 
\textbf{(1)} \textit{Recurrent} \citep{sanchez2018graph}: A recurrent model that also uses GRUs \citep{cho2014properties} to encode a history of interactions to infer system dynamics and perform system identification implicitly.
\textbf{(2)} \textit{MB-MAML} \citep{Nagabandi2019LearningTA}:  a model meta-trained using MAML, same as the one used for object pushing. It uses the same 16-step interaction trajectory for online adaptation.
\textbf{(3)} \textit{Expert-Ens}: An ensemble of separately trained experts, similar to the one used for object pushing. The only difference is that in pushing, we train one expert for each distinct object, while now we have a continuous distribution of terrain properties used for training. Therefore, for each task we pick several environments with properties evenly sampled from the continuous range, and train an expert for each of them.
\input{table_loco}

We apply all the methods with MPC for action selection and control, and report in Table \ref{table:loco} the average return computed over 500 episodes. Again, red numbers denote the best performance and the black ones represent the oracle performance. In all tasks, \HD\ is able to infer accurate system properties and generate corresponding dynamics models that match the oracle \textit{Expert-Ens} on seen terrains, and shows a great advantage over it when tested on unseen terrains. Our model also outperforms both \textit{MB-MAML} and \textit{Recurrent} on most of the tasks. Note that here \textit{Recurrent} can be viewed as serving the same sole of the \textit{Direct} baseline in pushing, since it feeds system features together with the states to a fixed global dynamics model. The results suggest that our explicit factorization of system features and the multiplicative way of aggregating it with low-dimensional state provide a clear advantage over methods that either train a fixed global model or perform online parameter adaptation on a meta-trained dynamics prior.


==> Intro.tex <==
\section{Introduction} \label{sec:intro}

Humans learn dynamics models that predict results of their interactions with the environment, and use such predictions for selecting actions to achieve intended goals \citep{Miall:1996:FMP:246663.246676,NIPS1998_1585}.  
These models capture intuitive physics and mechanics of the world and are remarkably versatile: they are  expressive and can be applied to all kinds of environments that we encounter in our daily lives,  with varying dynamics and diverse visual and physical properties.  
In addition, humans do not consider these models fixed over the course of interaction; we observe how the environment behaves in response to our actions
and quickly adapt our model for the situation in hand based based on new observations. 
Let us consider the scenario of moving an object on the ground. We can infer how heavy the object is by simply looking at it, and we can
then decide how hard to push. If it does not move as much as expected, we might realize it is heavier than we thought and increase the force we apply \citep{hamrick2011internal}.

Motivated by this, we propose {\em \HD}, a framework that  generates parameters for dynamics models (experts) dedicated to the situation in hand, based on observations of how the environment behaves.  The model has three main modules: i) an encoding module that encodes a few agent-environment interactions and the agent's visual observations into a latent feature code, which captures the properties of the dynamical system, ii) a hypernetwork \citep{ha2016hypernetworks} that conditions on the latent feature code and generates parameters of a dynamics model dedicated to the environment at hand, and iii) a target dynamics model constructed using the generated parameters that takes as input the current low-dimensional environment state and the agent action, and predicts the next  state, as shown in Figure \ref{fig:overview}.   We will be referring to this target dynamics model as an \textit{expert}, as it specializes on modelling the dynamics of a particular environment at a certain point in time.  \HD\ conditions on real-time observations and generates dedicated expert models on the fly. It is trained in an end-to-end differentiable manner to minimize state prediction error of the generated experts in each task and environment. 



\begin{figure*}[t]
\centering
		\includegraphics[width=0.8\textwidth]{figures/arch.png}
		\caption{\HD\ encodes the visual observations and a set of agent-environment interactions and generate the parameters of a  low-dimensional dynamics model for the current environment and timestep using a hypernetwork. \HD\ for pushing follows the general formulation, with a visual encoder for detecting the object in 3D  and encoding its shape, and an interaction encoder for encoding a small history of interactions of the agent with the environment.
		}
			\label{fig:overview}
			\vspace{-4ex}
\end{figure*}
 
  To place  HyperDynamics in the context of existing  literature on dynamics model learning and dynamics model adaptation we distinguish  five  groups of methods, depending on: i)  whether they explicitly distinguish between  dynamic properties---such as agent and object 3D or 2D locations and poses---and static properties---such as mass, inertia, 3D object shape--- of the environment,  ii) whether they update the dynamics model parameters or the static property values in the course of interaction, and iii) whether they consider visual sensory input  or operate on a predefined low-dimensional state representation. A method may belong to more than one categories. 
 Though such exposition is not  exhaustive, it will help us put the proposed work in perspective with existing methods. 
 
 
  \textbf{(i)} No adaptation with  low-dimensional state representations \cite{NIPS2018_7725}\todo{+++}.  These methods concern  dynamics models over low-dimensional states of the environment,  developed or learned for a specific environment. They cannot generalize across different physical properties of the same environment,  or across different environment.  
However, 
the low-dimensionality of their state facilitates forward unrolling, and these expert dynamics models are popular formulations in the literature.    
As a matter of fact, it has been shown recently that modelling epistemic and aleatoric uncertainty of such expert models during forward unrolling permits  model-based reinforcement learning formulations to surpass  model-free RL (in manipulating a single object or controlling a single environment) both in low- and high-data regimes \cite{NIPS2018_7725}. 


 \textbf{(ii)} System identification \citep{conf/eccv/BhatSP02}. These methods model explicitly the physical properties of the dynamical system using a small set of semantically meaningful physics parameters, such as mass, inertia, damping, etc. \citep{ajay,mrowca2018flexible}, and adapt their models across environment variations by learning their values  from data on-the-fly  \citep{chen2018hardware, li2018learning,  sanchez2018graph, battaglia2016interaction,pmlr-v80-sanchez-gonzalez18a}. 
 
 
 \textbf{(iii)} Recurrent state representations \citep{densephysnet,li2018push, ebert2018visual, sanchez2018graph}. These models learn to predict the next state from a history of state-action interaction  $s_{t+1}=f(s_{t-k},a_{t-k},...s_{t-1},a_{t-1};\phi)$, and 
%They do not explicitly separate static and dynamic properties of the system, and 
the recurrent hidden state implicitly captures information regarding the physical properties of the system.  They can operate over both high-dimensional visual observations or low dimensional state representations. These methods use a single and fixed global
dynamics model that takes system properties as input directly, together with its state and action.

%However, this can cause overfitting to the history of interactions if t
In this work we consider adaptation from a handful of interactions. Our visual object pushing task consider goals  as 3dimensional desired object locations, and is hard  to encode using only 2D images.

\textbf{(iv)} Online model adaptation via meta-learning \citep{DBLP:journals/corr/FinnAL17,Nagabandi2019LearningTA, clavera, DOMe}. These methods perform online adaptation on the parameters of the dynamics models through gradient descent. They are are optimized to produce a good parameter initialization that can be adapted to the local context with only a few gradient steps at test time.


\textbf{(v)} Visual dynamics and self-supervision \citep{DBLP:journals/corr/FinnL16, ebert2018visual, li2018push,xu2019densephysnet,DBLP:journals/corr/MathieuCL15, actionconditioned,DBLP:journals/corr/PathakAED17}.  These methods operate over high-dimensional images, and  learn their dynamics through frame prediction without any supervision of a state. Thus, they can adapt at test time to any environment assuming a very large number of interactions, to avoid overfitting \cite{ijcai2018-369}. In that respect, they are outside the scope of this work, since we consider adaptation from a handful of interactions. %, which is more realistic for real world systems. 



The expert models in \textbf{(i)} work well for their corresponding environments but fail to handle environment variations. A natural solution to address this is to train a separate expert for each environment. However, this approach does not scale and cannot transfer to environments with novel properties. 
Motivated by this need, 
%HyperDynamics learn a mapping between  how an environment looks and behaves to its low-dimensional dynamics transition function, % i.e., the mapping from states and actions $(s_t,a_t)$ to the next states $s_{t+1}$ or next state difference $\delta s_{t+1}$, 
%where the state contains only fast changing---such as agent and object 3D or 2D locations. 
% Similar environments will have similar corresponding dynamics functions. HyperDynamics attempt to exploit this regularity and learn such commonalities across different environments, or within the same environments across different timesteps. 
\HD\ learn a mapping between  how an environment looks and behaves to its low-dimensional dynamics expert model.  %HyperDynamics attempt to exploit this regularity and learn such commonalities across different environments, or within the same environments across different timesteps. 
Methods in (ii) and (iii), though attempt to infer system properties, optimize a single and fixed global dynamics model, which takes as input both static system properties and fast-changing states, with the hope that such a model can generalize across environment variations. 
 HyperDynamics instead of learning a global model that would work across any variation, instead learn a mapping from the environment behaviour and appearance to its ''local" low-dimensional dynamics.  Similar environment behaviours and appearances will have similar corresponding local dynamics models, and HyperDynamics  try to exploit this regularity and learn such commonalities across different environments, or within the same environment across different timesteps. 




 
 
 

We evaluate HyperDynamics on single- and multi-step state predictions, as well as  downstream model-based planning and control tasks.  Specifically, we apply it in a series  of object pushing and locomotion tasks across varying environments. Our experiments show that \HD\ is able to generate  dynamics models that match the performance of separately and directly trained experts, while also enabling effective generalization to environments with novel properties in a few-shot manner, outperforming representative models from the categories discussed above. We attribute its performance gain to the multiplicative way of combining explicit factorization of encoded system features with the low-dimensional state representation of the system. 
To the best of our knowledge, this is the first work that considers hypernetworks for adapting dynamics models. %We show through exhaustive ablations the benefits of the proposed methods, which we attribute to the multiplicative way of the history interaction  and visual context with the low-dimensional state representation of the environment and the agent. We further discuss implementation details that were crucial in getting the hypernetwork neural generation to work robustly, and we will share our datasets and code to stimulate research in this direction. 



==> Old_introsept28.tex <==
\section{Introduction} \label{sec:intro}

%When humans manipulate objects or interact with the world, they can generally predict how the world will change as a result of their actions.
%Such predictions are possible thanks to the multiple models of the world's dynamics that the human brain possesses, which are

Humans learn model of world dynamics through experience that predict results of their interactions with the environment, and use their predictions for selecting actions to achieve intended goals \cite{}. 
These models capture intuitive physics and mechanics of the world
%, geometry, affordance, and agent-object interactions. % regarding how the world works and reacts to agent's actions. %These models are learnt and continuously updated based on our experiences \citep{ha2018worldmodels}.  
%These {\em world models} 
 and are remarkably versatile: they are very expressive and can be applied to all kinds of scenes and environments that we encounter in our daily lives, with varying visual and physical properties.  
In addition, these models are not fixed over the course of interaction; we observe how objects behave
and quickly adapt our model for the situation in hand based on new observations. 
Let us consider the scenario of moving an object on the ground. We can infer how heavy the object is by simply looking at it, and we can
then decide how hard to push. If it does not move as expected, we might realize it is heavier than we thought and increase the force we apply.


Motivated by this, we propose {\em HyperDynamics}, a model that  generates parameters for low-dimensional dynamics models (experts)  based on observations of how the system behaves. 
Given a scene with certain properties, HyperDynamics networks observe its  response to a few interactions and potentially to its visual appearance, and automatically generate parameters of a dynamics model dedicated to the observed system, as shown in Figure \ref{fig:overview}. This dynamics model then takes as input the current system state (agent configuration and 3D object locations) and the agent action, and predicts the next system state. The model then takes the predicted state as input, and can optionally generate a new expert dynamics model, adapted to the recent history of interactions and visual observations.  
%In the predicted state, the model 


\todo{choices: newtonian system+system identification, MLPs+physical parameters estimated on the fly through fitting, MLPs MALM like, recurrent state represent, }


Learning dynamics  models that can generalise across environment physical and visual variations  is an open research problem whose solution would revolutionize model-based reinforcement learning, the field that investigates action selection by temporal unrolling of dynamics \cite{}.  
Consider the system of Figure \ref{} whose dynamics we are interested in learning.  A system is characterized by fast changing (dynamic) properties, such as agent and object 3D or 2D locations and poses, and slow changing (static) physical properties, such as mass, inertia, 3D object shape (during rigid interactions) and so on. 
 Given a  representation of the environment's and agent's state, learning dynamics is a supervised learning problem of mapping states and actions $(s_t,a_t)$ to the next states $s_{t+1}$ or next state difference $\delta s_{t+1}$. Methods vary regarding i) they explicit separate dynamic and static properties of the system, ii) learning dynamics using visual input or a predefined low-dimensional state, iii) adapting the dynamic model parameters versus adapting a small number of static property values.  To place our model in the context of recent literature, we group methods on learning dynamics and adapting them during the course of interaction into the following groups. Though such exposition may not be exhaustive, it helps us  place hyper-dynamics in the context of previous model learning and model adaptation methods:
 
 %A system is characterized by fast changing (dynamic) properties, such as agent and object 3D or 2D locations and poses, and slow changing (static) physical properties, such as mass, inertia, ... 

 i) System identification \cite{}. These methods capture the static properties of the dynamical system of the scene using a small set of physics parameters, such as mass, inertia, ..., and  learn/finetune their values  from data on-the-fly,  a procedure called system identification \cite{}. This process has been used both with Newtonian system of equations of motion, where domain knowledge is used for the structure of dynamics of the system, often used in control of air vehicles, \cite{}, as well as learning such dynamics mapping with machine learning models, such as MLPs \cite{} or graph neural networks \cite{}. %, where the equation structure is provided by domain knowledge and only few parameters are learnt from data.
 %The Physical laws are common across environments, and these methods  and do incorporate their physical properties such as mass, inertia, ..and shape and texture variability. Many dynamics models in control of follow such Newtonian dynamics equations \cite{}, and estimate values of physical parameters or object shapes from data, a procedure called system identification \cite{}, where the equation structure is provided by domain knowledge and only few parameters are learnt from data.
 %There are numerous research threads on learning 
 

 
 
ii) Recurrent state representations. These models learn to predict the next state from a history of state-action interaction  $s_{t+1}=f(s_{t-k},a_{t-k},...s_{t-1},a_{t-1};\phi)$. They do not explicitly separate static and dynamic properties of the system, and the recurrent hidden state captures information regarding the physical properties of the system. %update implicitly learns to adapt the the changing behaviour of the %rather they infer a recurrent state prediction rule, that 

iii) Online model adaptation through  gradient descent \cite{}. These methods adapt the dynamics model on the fly by finetuning it at test time \cite{}. However, this can cause overfitting to the history of interactions.

iv) Online model adaptation through meta-learning gradient descent optimization. These methods consider dynamics models and adapt all their parameters (as opposed to a small set of physic properties) through gradient descent. The model is optimized so that few gradient steps will generate a model that can adapt well in the test scenario, as opposed to overfitting in the interactions. 



 i) Dynamics learnt from high-dimensional sensory history observations. These are methods that take the raw sensory input in terms of a history of 2D images and  agent's state and predict a representation for the sensory input for the next time step,  such as a future image  , image embedding from which an image will be reconstructed, object 2D locations from which a future image can be generated \cite{}. In the state inferred there is no explicit separation of static and dynamic properties. These methods rely on recurrence of the visual information to adapt the dynamics mappings over time. %Most of those methods do not adapt the dynamics over time, 


%  Yet, the system of Newtonian dynamics equations is too complex to solve under contacts  for any other than the simplest environment. Thus,  researchers have tried to instead learn also the structure of the dynamics mapping from data offline or online during the course of interaction. For example, physical properties such as mass and friction are concatenated such (static) properties of the system with the fast changing state representation, such as agent 3D joint locations and object 3D locations and poses \cite{}, in MLPs or graph neural networks (Figure \ref{fig:intro}). Physical properties are estimated from data through gradient descent on the fly. 
%,  and adapt them through the course of interaction. %A central question here is the state representation. 
%Many works use  low dimensional state parametrization of the agent and its environment, such as agent 3D joint locations and object 3D locations and poses \cite{} (Figure \ref{fig:intro}). Physical properties that  Given a state representation, learning dynamics is a supervised learning problem of mapping states and actions $(s_t,a_t)$ to next states $s_{t+1}$ or the different $\delta s_{t+1}$ of the state.  Others, try to learn a state representation directly from the interaction history through recurrent state representations. 


%Many researchers have tried building high dimensional dynamics models over image visual input directly, and learn dynamics of images,  image embeddings or point/particle clouds conditioned on actions or interaction history. The high-dimensionality of the state makes this challenging, and the 2D nature of images challenges generalization across viewpoints.


%Others, consider low-dimensional dynamics over 3D locations of objects, or only over the agent's pose. Given that visual and interaction history are not part of the state representation in this case, a natural solution  is to train a separate dynamics  model, that specializes in each scenario, in other worlds, it is an experts for a a particular visual and interaction context, as shown in Fig. \ref{fig:intro}. However, this can hardly scale with the  number of systems, and is not able to transfer to system with novel properties. \todo{what about emta learning} So we  wonder, can we automatically generate an expert on the fly, by simply observing how a system behaves? Meanwhile, can such capability of \textit{generating experts} generalize to systems with novel properties not encountered during training? 
%for each dynamical system. % and try to adapt those based on visual observations and interaction history.  Since 3D object location

%For example, MALM
%These high dimensioanlThis has proven to be a very 


%World models enable humans to plan actions in order to achieve intended goals. The fields of model-based reinforcement learning (MBRL) and  trajectory optimization resemble this  mechanism of model-predictive action selection. They focus on developing models that predict the next state of a dynamical system given its current state and an agent action. These models are then unrolled forward in time for evaluating and choosing action sequences that achieve long term goals. However, many contemporary model-based approaches assume a fixed system without considering potential change in the underlying dynamics, and train a fixed dynamics model \cite{watter2015embed, banijamali2018robust, Fragkiadaki2015LearningVP,   zhang2019solar}. Such \textit{expert} models tend to fail when the system behavior changes. 

%A natural solution to address this is to train a separate expert for each dynamical system. However, this can hardly scale with the  number of systems, and is not able to transfer to system with novel properties. 



%Acquiring expressive and generalizable dynamics models has turned out to be a notoriously hard problem. Most prior works in this area propose methods that condition on system properties \cite{chen2018hardware, li2018learning, sanchez2018graph}, especially in the context of modeling  interactions with objects \cite{DBLP:journals/corr/FinnL16,agrawal2016learning, li2018push,xu2019densephysnet, battaglia2016interaction}, with the hope that the learned model  can transfer to novel systems. However,  many approaches use low-dimensional engineered state representations (such as explicit or estimated pose, mass and friction) \cite{chen2018hardware, li2018learning,  sanchez2018graph, battaglia2016interaction}, bypassing  high-dimensional visual input. These models cannot generalize across environments since the visual properties of the system are not taken into account. 
 %Other methods condition on visual inputs, and pass system information and states directly into a single dynamics model \cite{li2018push, xu2019densephysnet, DBLP:journals/corr/FinnL16, agrawal2016learning}, with the hope that it can handle varying system properties and transfer  acquired knowledge to  novel  systems. We argue that the way these models incorporate the additional system information that encodes system properties are inefficient. Specifically, this information is a representation of the system properties that may vary across different settings, and each instance of this representation ideally should correspond to a different dynamics model---an {\em expert}---that needs to be used in the corresponding setting. 
%The experts themselves can be simple models; each of them is a dynamics model targeted at a single fixed system.
%However, they share a lot of information as similar systems will have similar corresponding experts. Prior work does not explicitly consider this ``local'' structure and instead attempts to learn a single global model that receives the system features as an additional input. If such a model is trained on a small number of systems, it cannot generalize well to new ones because it does not make any explicit assumptions about the relationships between these systems.


Hyper-dynamics adapts all model's parameters based on interaction history and visual context, similar to methods in ((i),(ii)) but it generates  parameters for the dynamics model through a hypernetwork as opposed to gradient based optimization. The low-dimensional state representation of the generated dynamics model only captures fast changing dynamic state, similar to methods in (). It can condition on high-dimensional visual information as in the object-centric models of \cite{}. Specifically, we use a 3D object detector   to localize the object in 3D and feed its 3D feature map to the hypernet to generate parameters for a dynamics model that operates over the 3D object location and agent configuration and predicts future 3D object location and orientation, and 3D agent's configuration. 
Then, the 3D feature map is oriented to predict the paraneters of the model in the enxt timestep.  
%Interestingly we found %.  the object's appearance to condition on, and use a 3D object detector  

%We use 3D object detectort to infer this low-dimensinal state


We evaluate HyperDynamics its performance for single- and multi-step motion prediction, as well as for using the learned model for downstream planning and control tasks.  We apply it in the tasks of.  and compare with representative models from categories I,ii,iv and iv, showing superior performance. We further evaluate HyperDynamics in the visual task of  pushing diverse objects to different locations on the table surface, and compare against representative models in i,ii, showing better generalization to novel objects and camera viewpoints.
%as well as handlign camera viewpin
%the context of modeling object pushing. 
%We evaluate 
%Our experiments show that with only a handful of distinct objects used for training, HyperDynamics is able to match the performance of separately and directly trained experts, while also enabling effective generalization to objects with novel properties in a few-shot manner, addressing the aforementioned limitations of existing approaches.
%Note that, even though we only consider the setting of object pushing in the scope of this paper, the proposed HyperDynamics framework is general and \textit{potentially} applicable to a wide range of dynamics learning tasks, as we discuss in Section \ref{sec:conclusion}.
To the best of our knowledge, this is the first work that considers hypernetworks for dynamic adaptation. We show through exhaustive ablations the benefits of the proposed methods, which we attribute to the multiplicative way of the history interaction  and visual context with the low-dimensional state representation of the environment and the agent. We further discuss implementation details that were crucial in getting the hypernetwork neural generation to work robustly, and we plan to share our datasets and code to stimulate research in this direction. 

In summary, the main contribution of this work is to introduce hypernetworks for adaptation of dynamics models to visual context and to history of agent-environment interactions, and show that this model outperforms alternative adaptation strategies, as well as visual dynamics models build over 2D or 3D visual information directly. Importantly, we do not assume the state of the object known in the visual task, rather use a 3D detector and 3D feature representation for conditioning, that can handle varying camera placements, by exploiting camera extrinsics.  %that separates context from fast changign visual state.  %factorization of information, slow  some used for conditioning and some for

%to factorize observations into visual sensory and interaction  input used for parameter prediction and low-dimensional object and agent input used by the predicted dynamics expert for model-based control.  We propose a 3D feature representation for objects that can be used for conditioning---independent of the camera viewpoint--- as well as 3D object pose inference. Our code and datasets will be made publicly available upon publication.


%that we propose a general framework that is able to generate  expert dynamics models on the fly, conditioned on system features, and apply it to  the context of object pushing.
%We show that our approach matches performance of separately and directly trained experts, while also being able to transfer well to novel objects.

%In addition, we also show that our model outperforms alternative formulations which feed object features (both visual and physical properties) directly into a global dynamics model, as what most prior works do. Our code and datasets will be made publicly available upon publication.


==> note_intro.tex <==
\section{Introduction} \label{sec:intro}

Humans learn dynamics models that predict results of their interactions with the environment, and use their models' predictions for selecting actions to achieve intended goals \cite{Miall:1996:FMP:246663.246676,NIPS1998_1585}.  
These models capture intuitive physics and mechanics of the world 
 and are remarkably versatile: they are  expressive and can be applied to all kinds of environments that we encounter in our daily lives, that may wildly vary in their physical  properties and visual appearance.   
In addition, humans do not consider these models fixed over the course of interaction; we observe how objects behave
and quickly adapt our model for the situation in hand based on new observations. 
Let us consider the scenario of moving an object on the ground. We can infer how heavy the object is by simply looking at it, and we can
then decide how hard to push. If it does not move as expected, we might realize it is heavier than we thought and increase the force we apply \cite{hamrick2011internal}.

\begin{figure*}[t]
	\centering
		\centering
		\includegraphics[width=\textwidth]{figures/arch.png}
		\caption{\todo{place holder figure, i'll replace it}}
			\label{fig:overview}
\end{figure*}


 
 
Motivated by this, we propose {\em HyperDynamics}, a model that  generates parameters for low-dimensional dynamics models (experts)  based on observations of how the environment behaves. HyperDynamics has two modules: i) a hypernetwork \cite{ha2016hypernetworks} that conditions on a few  agent-environment interactions and visual object appearance and generates parameters of a dynamics model dedicated to the observed system, and ii) a target dynamics model whose parameters are generated  that takes as input the current system state (agent configuration and 3D object locations) and the agent action, and predicts the next system state, as shown in Figure \ref{fig:overview}. The hypernetwork then takes the predicted state as input, and can optionally generate a new target dynamics model, adapted to the predicted states and visual appearances of the environment.  We will be referring to this target dynamics model as an expert, as it specializes on encoding the dynamics of a particular scene at a certain point in time, and cannot generalize across scenes.  
  HyperDynamics are trained in an end-to-end differentiable manner to minimize state prediction of the target generated networks in each task.



HyperDynamics learn a mapping between  how a scene looks and behaves to its low-dimensional dynamics function,  i.e., the mapping from states and actions $(s_t,a_t)$ to the next states $s_{t+1}$ or next state difference $\delta s_{t+1}$, where the state contains only fast changing---such as agent and object 3D or 2D locations. 
 Similar systems will have similar corresponding dynamics functions. HyperDynamics attempt to exploit this regularity and learn such commonalities across different systems, or within the same system across different timesteps. 
 
 
 %Prior work does59not explicitly consider this “local” structure and instead attempts to learn a single global model that60receives the system features as an additional input. If such a model is trained on a small number of61systems, it cannot generalize well to new ones because it does not make any explicit assumptions62about the relationships between these systems.


%Though the world may look and feel complex, its dynamics,


%and not slow changing (static) physical properties, such as mass, inertia, 3D object shape (during rigid interactions)

%propertiesIn general, a system is characterized by fast changing (dynamic) properties, such as agent and object 3D or 2D locations and poses, and slow changing (static) physical properties, such as mass, inertia, 3D object shape (during rigid interactions) and so on.  

%Specifically, this54information is a representation of the system properties that may vary across different settings, and55each instance of this representation ideally should correspond to a different dynamics model—an56expert—that needs to be used in the corresponding setting. The experts themselves can be simple57models; each of them is a dynamics model targeted at a single fixed system. However, they share58a lot of information as similar systems will have similar corresponding experts.  Prior work does59not explicitly consider this “local” structure and instead attempts to learn a single global model that60receives the system features as an additional input. If such a model is trained on a small number of61systems, it cannot generalize well to new ones because it does not make any explicit assumptions62about the relationships between these systems.

%Hyperdynamics are based on the intuition that though the environment may look and feel complex, few things only can change over time, and whose dynamics we care to learn to predict the future. Consider the scene in Figure \ref{} whose dynamics we are interested in learning. It contains a complex looking object but the appearance of the object will remain constant over time in 3D, same goes for its physical properties such as its mass and % For example, we may have a very complex 

% In general, a system is characterized by fast changing (dynamic) properties, such as agent and object 3D or 2D locations and poses, and slow changing (static) physical properties, such as mass, inertia, 3D object shape (during rigid interactions) and so on. Hyperdynamics condition on visual context and history of interaction to implicitly infer physical and shape properties for the system and predict the parameters that dictate the dynamics of its fast-moving state, such as 3D location and agent configuration
 
 %Given a  representation of the environment's and agent's state, learning dynamics is a supervised learning problem of mapping states and actions $(s_t,a_t)$ to the next states $s_{t+1}$ or next state difference $\delta s_{t+1}$. 
 
 %Research methods vary regarding  
 
 
 %To place the proposed HyperDynamics in the context of recent literature, 
 To place  HyperDynamics in the context of existing  literature on model learning and adaptation, we distinguish  four  groups of methods, depending on  whether they explicitly distinguish between  dynamic---such as agent and object 3D or 2D locations and poses---and static ---such as mass, inertia, 3D object shape---properties of the system,  whether they update the dynamics model parameters or  the static property values in the course of interaction, and  whether they consider visual sensory input  or operate on a predefined low-dimensional state representation. 
 Though such exposition may not be exhaustive, it will help us put the proposed work in perspective with existing methods. %understand the  place the proposed HyperDynamics in the context of recent literature:
 
 %A system is characterized by fast changing (dynamic) properties, such as agent and object 3D or 2D locations and poses, and slow changing (static) physical properties, such as mass, inertia, ... 


\textbf{(i)} Mixture of expert models. These methods maintain a pool of models and select the fittest one at test time  using few interactions, often using Bayesian optimization to balance. 


\textbf{(i)} No model adaptation \cite{}. 
In this group, we consider: a) dynamics model over low-dimensional states of the system. They are developed/learned for a specific system and cannot generalize across different  physical properties of the same system,  or across different systems \cite{}. b) Dynamics model over high-dimensional sensory observations, such as images or 3D pointclouds \cite{}. These  methods infer a low-dimensional state of the system  from a history of 2D images or 3D poinclouds \cite{li2018push, xu2019densephysnet, DBLP:journals/corr/FinnL16, agrawal2016learning} and predict a representation for the sensory input for the next time step,  such as a future 2D image \cite{DBLP:journals/corr/FinnGL16,DBLP:journals/corr/FinnL16,ebert2018visual,actionconditioned,DBLP:journals/corr/abs-1710-05268,NIPS2015_5859,DBLP:journals/corr/abs-1903-00374}, image embedding from which an image will be reconstructed \cite{hafner2019planet}, object 2D locations from which a future image can be rendered \cite{DBLP:journals/corr/abs-1812-10972,Fragkiadaki2015LearningVP}. In the state inferred there is no explicit separation of static and dynamic properties. 



 \textbf{(i)} System identification \cite{conf/eccv/BhatSP02}. These methods model explicitly the static properties of the dynamical system  using a small set of semantically meaningful physics parameters, such as mass, inertia, .... \cite{ajay,mrowca2018flexible}, that are hard to discern visually. They  learn/finetune these values  from data on-the-fly  \cite{chen2018hardware, li2018learning,  sanchez2018graph, battaglia2016interaction,pmlr-v80-sanchez-gonzalez18a,} \todo{we need 4-5 traditional robotics works here that use Newtonian equations}. This process has been used both with Newtonian system of equations of motion, where domain knowledge is used for the structure of dynamics of the system, often used in control of air vehicles, \cite{}, as well as learning such dynamics mapping with machine learning models, such as MLPs \cite{} or graph neural networks \cite{battaglia2016interaction, li2018learning}. 


\textbf{(ii)} Recurrent state representations \cite{pushnet}. These models learn to predict the next state from a history of state-action interaction  $s_{t+1}=f(s_{t-k},a_{t-k},...s_{t-1},a_{t-1};\phi)$. They do not explicitly separate static and dynamic properties of the system, and the recurrent hidden state captures information regarding the physical properties of the system. 

\textbf{(iii)} Online model adaptation \cite{} and self-supervised model learning through  gradient descent \cite{densephysnet, DBLP:journals/corr/FinnGL16,DBLP:journals/corr/FinnL16,ebert2018visual,actionconditioned,DBLP:journals/corr/abs-1710-05268,NIPS2015_5859,DBLP:journals/corr/abs-1903-00374}. These methods adapt the dynamics model on the fly by finetuning it at test time \cite{ijcai2018-369}. However, this can cause overfitting to the history of interactions if the model capacity is high, and has been used effectively with low-dimensional local models \cite{fu}.

\textbf{(iv)} Online model adaptation through meta-learning gradient descent optimization \cite{DBLP:journals/corr/FinnAL17,Nagabandi2019LearningTA,clavera}. These methods consider dynamics models and adapt all their parameters (as opposed to a small set of physic properties) through gradient descent. The model is optimized so that few gradient steps will generate a model that can perform well in the test scenario, as opposed to overfiting to the small set of interactions, by backpropagating through the gradient descent optimization process.  




%Dynamics learnt from high-dimensional sensory history observations. These are methods that take the raw sensory input in terms of a history of 2D images and  agent's state \cite{li2018push, xu2019densephysnet, DBLP:journals/corr/FinnL16, agrawal2016learning} and predict a representation for the sensory input for the next time step,  such as a future image \cite{}, image embedding from which an image will be reconstructed, object 2D locations from which a future image can be generated \cite{}. In the state inferred there is no explicit separation of static and dynamic properties. These methods rely on recurrence of the visual information to adapt the dynamics mappings over time. 


HyperDynamics adapts all model's parameters based on interaction history and visual context, similar to methods in ((i),(ii)) but it generates  parameters for the dynamics model through a hypernetwork as opposed to gradient based optimization. The low-dimensional state representation of the generated target dynamics model only captures fast changing dynamic state, similar to methods in (). Static properties are not explicitly represented rather implicitly inferred through conditioning on recent history of interactions, like recurrent models in (), It can condition on high-dimensional visual information as in the object-centric models of \cite{}. Specifically, we use a 3D object detector  to localize the object in 3D and feed its 3D feature map to the hypernetwork to generate parameters for a dynamics model that operates over the 3D object location and agent configuration and predicts future 3D object location and orientation, and 3D agent's configuration.  Then, the 3D feature map is oriented to predict the parameters of the model in the next timestep.  


We evaluate HyperDynamics on single- and multi-step state prediction, as well as  downstream model-based planning and control tasks.  Specifically, we apply it in the tasks of.  and compare with representative models from categories I,ii,iv and iv, showing superior performance. We further evaluate HyperDynamics in the visual task of  pushing diverse objects to different locations on the table surface, and compare against representative models in i,ii, showing better generalization to novel objects and camera viewpoints. 
To the best of our knowledge, this is the first work that considers hypernetworks for adapting dynamics models. We show through exhaustive ablations the benefits of the proposed methods, which we attribute to the multiplicative way of the history interaction  and visual context with the low-dimensional state representation of the environment and the agent. We further discuss implementation details that were crucial in getting the hypernetwork neural generation to work robustly, and we will share our datasets and code to stimulate research in this direction. 




\section{Introduction} \label{sec:intro}


\topic{what humans can do: they adapt dynamic models on the fly}

Humans predict how the world will change as a result of their actions and interactions.   Such predictions are possible thanks to the multiple models of the world's dynamics the brain possesses that are learnt and continuously updated  with experience \cite{wolpert}. We use models to plan actions and achieve intended goals.  Such models are remarkably versatile: they are both very expressive and are applied to all kinds of systems we encounter in our daily lives, with varying dynamics, diverse appearances and physical properties. In addition, such models  are not fixed over the course of interaction; we observe how objects behave and quickly adapt our models based on new observations \cite{}. Let us consider the scenario of moving an object on the ground. We can infer how heavy the object is by simply looking at it, and we can then decide how hard to push.
%We can infer how heavy it  is and how much force we need to exercise by the object's appearance.  \todo{roll and push are kind fo the same...}%We might even adapt our strategy and decide to go  with rolling instead of  pushing if it  is  a  sphere,  just to reduce our effort.
%If it does not move as much as we expected, we realize it's heavier than  we thought and  increase  our force, or even engage both hands.
If it does not move as expected, we might realize it is heavier than we thought and increase the force we apply.

%Such predictive models allow us to plan actions in  order to achieve intended goals,
\topic{machines try to do model-based control  with MBRL}

The fields of model-based reinforcement learning (MBRL) and  trajectory optimization,  both are inspired by the model predictive action selection in the human brain.
They are both focused on developing models that, in their simplest form, predict the next state of  a dynamical system  given its current state and  action. These models can be learned from data or be engineered. They are then unrolled  forward in time and are used for optimization for action sequences that achieve long term goals. 


 %Model-based Reinforcement  Learning (RL) algorithms  resemble this mechanism: a dynamics model learns to predict how a dynamical system behaves given current state and action, and is then unrolled forward in time for downstream planning and control tasks. However, many contemporary model-based approaches assume fixed systems with constant physical properties, and train a separate model dedicated to each system \cite{watter2015embed, banijamali2018robust, Fragkiadaki2015LearningVP,   zhang2019solar, hafner2019planet}. Such \textit{expert} models are tied with  fixed systems and tend to fail when the system behavior changes. A natural solution to address this is to train a separate  expert for each dynamical system. However, training such an ensemble of experts could be computationally impractical when the  number of systems grows, and it's also difficult for  them to transfer to system with novel properties not encountered  during training. So we  wonder,  can we have a model that is able to automatically generate an expert on the fly, by simply observing how the system behaves? Meanwhile, would it be possible for such capability of \textit{generating experts} generalize to systems with novel properties not encountered during training?

\topic{model learning is hard, approaches on model learning}
Acquiring expressive and generalizable dynamics models for object interactions has turned out to be a notoriously hard problem, despite its supervised nature \cite{}. The research directions in interaction model learning can be split into two main categories: i)    Models that condition  on visual observation streams  \cite{chen2018hardware, li2018learning, sanchez2018graph,DBLP:journals/corr/FinnL16,agrawal2016learning, li2018push,xu2019densephysnet, battaglia2016interaction}, with the hope that the learned model  can transfer to novel interactions, scenes or camera viewpoints. ii)  Models that use low-dimensional engineered object state representations (such as explicit or estimated 3D object centroids, poses, mass and friction) \cite{chen2018hardware, li2018learning,  sanchez2018graph, battaglia2016interaction}, bypassing  high-dimensional visual input. The former suffer from the difficulty in predicting visual dynamics, and have not been found to effectively generalize across environment dynamics or changes of the camera viewpoint \cite{}. The later essentially give up on generalization across scenes  since the visual properties of the objects are not taken into account. %Such {\em expert} models are tied to the fixed systems they are trained for and tend to fail when system behavior changes.
%They are like an ``expert" model that captured the dynamics of a specific object/scene configuration, they are tied to the fixed systems they are trained for and tend to fail when system behavior changes, e.g., the object shape changes. 
%Yet, they are more successful than models over high dimensional observations \cite{}, as training predictive models over low-dim observations is dramatically easier that using visuals. 
%and competitive to model free RL moth in low number of examples as well as ay
%Yet, they ioften perform better since predictive 
%Such \textit{expert} models are tied with  fixed systems and tend to fail when the system behavior changes. A natural solution to address this is to train a separate  expert for each dynamical system. However, Training such an ensemble of experts could be computationally impractical when the  number of systems grows, and it's also difficult for  them to transfer to system with novel properties not encountered  during training.
%Our work asks the following questions: 
%Can we automatically generate  low-dim dynamics expert models on-the-fly, by simply observing how the environment looks and responds to agent interactions? Meanwhile, would  this capability of \textit{generating expert dynamics} generalize to systems with novel properties (visual or physics) not encountered during training?



 
To this end, we propose \textit{HyperDynamics}, a model that
using high-dimensional visual observations of a system and its responses to agent actions to generate on-the-fly parameters for a dynamics model  over a low-dimensional representation of the system in hand. %Given a system with certain properties, HyperDynamics networks observe its visual appearance and/or response to a few interactions, and automatically generate dynamics models dedicated to the observed systems.
%extends the current family of model-based RL methods by incorporating the capability of `\textit{automatic expert generation}'. 
%Given a system with certain properties, our method observes its visual appearance and/or response to a few interactions with it, and generate a dynamics model dedicated to the observed  system on the fly. 
The generated  dynamics model is a neural network that takes as input the system's low-dim state representations, e.g., an object's and gripper's  centroids and  action given by the agent, and  predicts the system's change of state in the next timestep. 
We evaluate HyperDynamics in the context of modelling object pushing with a diverse set of obejcts. 
Specifically, we evaluate performance for single- and multi-step motion prediction, and for using the learned dynamics model for downstream planning and control tasks.
As we shall show, HyperDynamics enable generalization to objects with novel visuals and physics properties not encountered during training, while also being able to scale well as the number of objects grows, addressing both aforementioned limitations of existing approaches. %It emulates the performance of expert models trained for each object independently, can generalize beyond the training set, and outperforms baselines that use the visual observations of the system as input to the dynamics model directly. 


%The model's predictions are unrolled over time by concurrently warping the visual input using the predicted change of state, and re-generating dynaics model to be applied to the predicted visual appearance of the objects. 
%Importantly, we use a 3-dimensional visual representation for the objects, which can be easily warped based on predicted motion, to generate future visual states for the system. 



 

Our contributions are as  follows:

 \begin{itemize}
\item  We propose a general framework that is able to generate  dynamics model on the fly, conditioned on system visual observations and responses to agent actions, and apply   it to  the context of object pushing.
\item We show our approach matches performance  of separately and directly trained experts, while also being able to transfer well to  novel objects  in a zero-  or  low-shot manner.
\item We show  our model outperforms alternative formulation that feeds object features (both  visual and  physical properties) directly  into a unified  dynamics model, as what most methods in the current literature do.


  \end{itemize}
  
Our code and datasets will be made publicly available upon publication.
 
 
 

==> note_model.tex <==
\section{HyperDynamics for Object Pushing}
\label{sec:model}

\todo{Hyper-dynamics as model name}

\begin{figure*}[t]
	\centering
		\centering
		\includegraphics[width=\textwidth]{figures/arch.png}
		\caption{\todo{place holder figure, i'll replace it}}
			\label{fig:arch}
\end{figure*}


We consider a robotic agent equipped with an RGB-D camera to observe the world and an end-effector to interact with it. The goal of the agent is to push objects to desired locations on the table surface. Objects can vary in their shape, appearance and their physics properties, such as mass and friction with the table surface.  
Our contribution is a novel model learning scheme where a hyper-network learns to predict weights for a dynamic network 
that can adapt to changing appearance and physics properties of the objects. We will then control objects to desired locations using standard model-predictive control, by unrolling the nyper-dynamics model forward in time. 


The architecture of Hyper-Dynamic Networks (HDNs) is illustrated in Figure \ref{fig:arch}.  
HDNs are comprised of two neural networks. A  \textit{hyper-network}   takes as input a
visual representation of the object 
in hand 
as well as its displacements to  a small set of agent actions and predicts neural weights for a second neural network,  which we will call the  \textit{dynamics expert}. The dynamics expert is a forward temporal dynamics model and takes as input a low-dimensional representation of the state of the object and the agent at time step  and the action of the agent, and predicts the next state for the object and the agent. 
The state of the object  purposefully does not include information regarding the visual appearance or physics properties of the object, since these properties do not change over time. Since visual appearance or physics properties are not modelled in any way, such dynamics models cannot possibly generalize across objects. We use thus the term expert object dynamic model to refer to a dynamic models trained for a specific object (i.e., an object with specific appearance, mass and friction).  Such expert dynamic models are popular formulations in the literature. As a matter of fact, recently, 
modelling epistemic and aleatoric uncertainty of such expert dynamics model during unrolling permitted  model-based formulation to surpass  model-free RL (in manipulating a single object or controlling a single system) both in few as well as in lots of training data regimes \cite{NIPS2018_7725}. Our framework  generalizes such formulation to handle any system by predicting their parameters using a hyper-network that does conditions on visual appearance and physics properties of the object in hand. The only difference is that instead of learning the weights of such expert dynamics models using SGD as in related works \cite{NIPS2018_7725}, we will be predicting them using the hyper-network. Weights of the hyper-network will be learnt via SGD by back-propagating the expert model prediction error in an end-to-end differentiable manner.  


We describe our expert dynamics model in Section \ref{sec:expert} and our hyper-network  in Section \ref{sec:hypernet}.
We discuss use of our hyper-dynamics for temporal unrolling and model-predictive control in Section \ref{sec:MPC}. Last, in Section \ref{sec:single}, we discuss inference of visual representation of the object from 2.5D single view images, as opposed to ground-truth. Note that the vast majority of prior works in modelling object pushing dynamics  consider only quasi-static pushing or poking, in which an object always starts to move or  stops together with the robot's end-effector \cite{DBLP:journals/corr/FinnL16, agrawal2016learning, li2018push, pinto2017learning}. We go beyond simple quasi-static pushing by wildly varying the physics parameters of the object and the scene, and allow an object to slide by itself if pushed with a high speed \todo{with large force?}. 



\subsection{Expert Object Dynamic Models}
\label{sec:expert}
%We first  describe  the  expert dynamic models in our  setting, since they serve as an important baseline for comparison. 

The expert dynamics model $\ff^o$ learn a (deterministic) mapping between the state of an object $\xx_t^{o}$ and the robot's gripper $\xx_t^{r}$ at timestep $t$ and action applied by the agent $\act_t$, to  the  state change at subsequent time step $t+1$, $\delta \xx_t = \ff^o(\xx_t, \act_t)$,  where $\delta \xx_t = <\delta \xx_t^{o}, \delta \xx_t^{r}>$ includes state change for both the object and the robot.  
%, though this is often 
%Yet, visual appearance or physics properties much determines the dynamics of an object% and thus we do not need to model their dynamics.
%$t$ $\xx_t$
The object state include object position, orientation, translational and rotational  velocities and the robot state \todo{??}
For controlling the robot, we use position-control in our experiments, so the action $\act_t = (\delta x, \delta y, \delta z)$ is a 3-vector representing the movement of the  robot's end-effector. Note that a PID controller controls the robot's torque in its joint  space under the hood, based on the  position-control commands, so varying the magnitude of the action could lead to different pushing speed of the end-effector. 
Given a pool of $N$ (training) objects and one robotic agent manipulating them, we will have a separate expert $\ff^o$ for modelling dynamics of each object. 

%In our setting, $\xx_t^{o}$ is a 13-vector containing the object's position $p_t^{o} \in \mathbb{R}^3$, orientation $q_t^{o} \in \mathbb{R}^3$ (represented as quaternion), as well as its translational and rotational velocities $v_t^{o} \in \mathbb{R}^6$. \todo{how it is 13?} %We have $\xx_{t+1}= \xx_t+ \delta \xx_t$. 
%$\delta x_t^{obj}$ is a vector with the same size representing the change in the object's position, orientation and velocity. The same applies to $x_t^{rob}$  and $\delta x_t^{rob}$. 


%We  train a ensemble of $N$ experts, one for each object,  and use them as a reference for experimental comparison.
%\subsection{Encoding Object Features}
%\label{sec:encoder}

\subsection{Generating Neural Weights for Expert Object Dynamics }
\label{sec:hypernet}

Our hyper-network takes as input information regarding the shape and the physics parameters of the object to predict neural weights that parametrize a corresponding expert dynamics model for that object.  
 %We consider both of those sets of observations as input to our hyper-network, to predict weights for expert dynamic models. 
The way objects move when pushed depends  
%Given an object $o$, its behavior under pushing is affected  by 
both on their 3D shape, as well as their physics properties, such as,  mass, friction, restitution, etc. . While 3D object shape can be inferred by visual observation,  the later physics properties  are hard to discern visually.  They can be inferred by observing the  motion of an object as a result to few (random) pokes from the robot \cite{xu2019densephysnet}. \todo{we may want to talk more about that citation}
Our hyper-network takes as input 3D binary voxel occupancy grid that represents the shape of the object, and its motion trajectory in few pokes, and predicts the expert dynamic model  parameters, as shown in Figure \ref{fig:arch}.  
%Though the representation itself  is agnostic to the object appearance and physics properties,   the generated weights are conditioned  and thus depend on such properties, which permits HDNs to generalize across objects's appearance and physics. 



Let $V^o \in \{0,1\}^{w \times h \times d}$ denote an object-centric binary  occupancy voxel grid. We will consider $V^o$ to be provided by an oracle for now, such as a simulator environment,  and discuss in Section \ref{sec:vision} how to infer this from RGB-D images using view prediction networks. A 3D convolutional encoder network $\Eshape$ maps  $V^o$ to a 1-dimensional feature code $z^o_{shape} \in \mathbb{R}^{50}$. \todo{?}
Let $\tau^o \in \mathbb{R}^{3 \times T_{inter}$ denote the object trajectory when pushed for $T_{inter}$ timesteps in random directions (\todo{different for each object?}) but same in magnitude. We found  $T_{inter}=5 $  sufficient  to yield good performance and used it in  all our experiments. 
A fully connected network $\Einter$ maps the trajectory to a 1-dimensional code $z_{physics}^o$ that represents information regarding the physical properties of the object (entangled). 
A hyper-network $\Eweight$ maps the concatenated code $z^o=[z^o_{shape},z^o_{physics}]$ to a set of neural network weights for the dynamics expert $\ff$  described in Section \ref{sec:expert}. 
\todo{XIAN: can you write details here? how many weights/ how do you predict those, whats the architecture? is is all at once that you predict them?}%%except that  its  weights are  not directly optimized, but produced  from the hypernet.
%Given the  object $o$, the robot will push it from random directions for $N_{inter}$ times. 
 

%These  pushing actions are random in direction but same in magnitude. We record a sequence of the  object's motions under these  pushes, and pass this record of interactions into the physics encoder, which produces another latent vector  $v^p_o$ encoding the object's physics properties such as its mass and friction coefficient.

%\subsection{Expert Generation Conditioned on Encoded Features}
%\label{sec:weights}
%By composing $v_o^g$ and  $v_o^p$ described above, we now have  a single vector $v_o$ encoding the object's  all properties relevant to pushing. 

%A hypernet module is in charge of generating an expert specific for object $o$. We feed $v_o$ into the hypernet, which returns all parameters needed for an  $o$-specific dynamics model $f_o$. This dynamics model shares the same architecture  and  purpose of the experts described in Section \ref{sec:expert}, except that  its  weights are  not directly optimized, but produced  from the hypernet. 

%\subsubsection{}
%In the architecture discussed so far, it seems  we already have a clear and intuitive  division of tasks among different modules: given a  object $o$, the encoder infers its property based on its appearance and some interactions with it; the hypernet generates a single dynamics model  for it; the generated dynamics model serves as an object-specific expert and predicts its motion under pushing given its full state. However, one important issue we need to address is generalization: we  want HyperDynamics to generalize to unseen objects even without seeing a  huge number of objects during training. With  the   architecture presented so far, when there's only a few objects in the training set, the hypernet will only be able to see very few data samples instead of a wide distribution of object features. Effectively, it's only trained to optimize a discrete set of dynamics models for motion prediction, thus potentially leading to severe overfitting on the training data. 

%In order to overcome  this, we propose a simple change to the aforementioned task divisions. 

We train our hypernetwork by backpropagating error gradients of the prediction of the generated network, all the way to our shape and physics encoders and weight generator.  
We also additional regularization losses by autoencoding the object's 3D shape, passing the 3D shape code  $z^o_{shape}$ to a convolutional decoder and minimizing a reconstruction loss. 
Let $\mathcal{O}$ denote the training object pool available. Let $T$ denote the length of an interaction trajectory. Let $N$ denote the number of trajectories per object. 
The final loss for HDNs reads:
\begin{equation}
    \mathcal{L}=  \frac{1}{|\mathcal{O}| T } \sum_{t=1}^T \sum_{o=1}^{|\mathcal{O}|}\underbrace{\|\xx^o_{t+1} - \ff(\xx^o_t,\act^o_t;\Eweight(z^{o,t}_{shape},z^o_{physics})) \|_2}_{\text{dynamics prediction}} + \underbrace{\|V^{o}_t- \Dshape(\Eshape(V^{o}_t)) \|_2}_{\text{shape autoencoding}}
\end{equation}

Note that the autoencoding loss can be applied in any object we have available, even objects not pushed by our agent. 


\paragraph{Object 3D orientation: context or state?}
%Permanent ---non changing over time--- object properties, such as its shape or friction and mass are used as content for the hypernetwork to predict neural parameters for a second neural network that  models the temporal dynamics of the properties of the object that are actually changing over time, such as, the object and gripper 3D location. 
The 3D shape of rigid objects does not change over time, rather, its 3D orientation changes. 
Should we use the canonical (non-oriented) 3D shape information as context for parameter prediction, in which case the 3D object pose (with respect to that canonical coordinate frame) would be used as part of the fast changing state $\xx^o$ in the experts dynamics model, or we should use the oriented 3D shapes context for parameter prediction, in which case the object pose is encoded in the weights of the expert dynamicas, and thus only the 3D object location is part of the fast changing state $\xx^o$. 
%Note that the voxel grid $V^o$ of the object at time step $t$ represents the  orientation of the object at time $t$, not the canonical (and thus time unaffected) orientation. 
Empirically, we found two benefits in feeding the oriented feature map $\M^o$ to the hyper-network and discarding object pose from the input of the expert dynamics network:
i) it would require supervision to define object canonical 3D orientation. It is unclear how to define a canonical orientation in an intuitive way for novel objects to permit HDNs to generalize.
ii) Using oriented as opposed to canonical shape as input, permits $\hn$ to have way more training examples, even from a small number of objects with distinct shape  pushed on the table. 
%If pose information would be part of the state input to f as opposed to h, then h would have very few training example to be trained on, since we 'd require a large number of distinct objects to be pushed in the simulator to learn it. 
%Instead of feeding voxel grids of the objects  with canonical poses and feeding the full state of the object to the generated dynamics model, we move the orientation information from the input of the dynamics model to the input of the hypernet. More specifically, when the object $o$ is at a certain orientation $q_o$, we re-orient it's voxel grid to match $q_o$ before feeding it into the geometry encoder, and simply discard the orientation information in the object's state that's fed into the generated dynamics model. As a result, the hypernet will be trained on feature vectors encoding objects with various orientations.
Intuitively, the hypernet  treats an object at different orientations as different objects, and generates different experts for each. This helps smoothen and widen the data distribution seen by the geometric feature encoder, and thus the hypernet, making the learning process much more sample-efficient. In addition, this also reduces burden for the  generated expert, as now it does not need to process orientation information.




\subsection{Inferring 3D object shape from RGB-D Images}
\label{sec:single}
So far  we assumed access to ground-truth 3D occupancy voxel grids to represent the 3D shape of an object. Such information is readily available  in simulation  but unavailable in the real-world. 
We learn to map single view depth maps (2.5D) to  complete  3D feature grids $\M \in \mathbb{R}^{w \times h \times d \times c}$ that represent the appearance and shape of the scene and its objects by training Geometry-Aware Recurrent Networks (GRNN) of \cite{commonsense} for cross-view depth prediction. GRNNs learn to map RGB-D (2.5D) images to complete 3D feature grids of the scene they depict using differentiable unprojection (2.5D to 3D) and projection (3D to 2.5D) neural modules and are optimized end-to-end but the task of view prediction. Their architecture uses biases regarding image formation and 3D geometry. Specifically,  the 3D feature map inferred from an input  view is oriented to the query viewpoint, and neurally projected to match the RGB-D image of the query view. In this way, they learn to complete information from  each view to infer a complete 3D feature grid. 
We apply GRNNs using only depth maps as input and as prediction output, and disregarding RGB information, since texture is less relevant to object pushing dynamics. 
%s information 
`%lift" a single RGB-D image to an incomplete voxel grid by placing voxel occupancies according to the input depth map. The voxel grid is passed through a 3D convolutional encoder , is oriented to a target viewpoint and decoded to a depth map from that view. Depth prediction is used to optimize the weights of the GRNN. In this way, the occupancy voxel grid is completed. Upon training, GRNNs can map a single image  to a full object-centric occupancy 3D grid for the scene it depicts. 
%
We crop the scene map using 3D object bounding box $b$ to produce an object-centric map  $\M^o=\mathjrm{crop}(\M,b)$, which we use as input to our hyper-net. 
We use 3D box information provided by the simulator at training time, and 
 train a 3D object detector, a modified Faster-RCNN \cite{} to map full scene feature maps $\M$ to a set of 3D bounding boxes for the objects present, following \cite{commonsense}, to be used at test time. 
%\todo{do you use an object detector?} Locations of the objects are produced from the jointly trained object detector, or can be estimated accurately using simple techniques such as background subtraction. 
%In practice, we follow the Geometry-Aware Recurrent Networks (GRNN) framework presented in \cite{commonsense}, to ``lift" a single RGB-D image to the 3D space in order to obtain a 3D object-centric representation of the object
%. Given a single RGB-D image $I$, GRNN learns to convert it to a 2D feature map and then project the feature map into the 3D space. It can be trained end-to-end for a downstream task, such as 3D  object detection or view prediction from novel viewpoints.
%GRNN can also be optimized to \textit{imagine} missing or occluded information, essentially learning shape completion from a single image input, which is very useful for our tasks. We refer readers to \cite{commonsense} for more details. In practice, after we obtain a 3D feature map of the scene, we crop around the object to get an object-centric 3D feature tensor $\M^o$. Locations of the objects are produced from the jointly trained object detector, or can be estimated accurately using simple techniques such as background subtraction. 

%Estimating orientation information has always been a hard problem for computer vision \todo{some citations?}, but explicit estimation is not needed in our framework due to its implicit way of encoding orientation using the object feature vector, as discussed above.



\subsection{Model unrolling and Model Predictive Control }
\label{sec:MPC}
Action-conditioned dynamics model can plan by  forward in time unrolling and be used for action selection and control tasks. The unrolling mechanism of HDNs is straightforward: at each timestep $t$, a generated dynamics model $\ff^{t)}$ predicts $\delta \xx_t$. Afterwards, we compute $\xx_{t+1} = \xx_t \oplus \delta \xx_t$, where $\oplus$ represents simple summation for positions and velocities, and quaternion composition for orientations. We then re-orient the 3D object-centric feature map $\M^o$ using the updated orientation $q_{t+1}$ and generate a new dynamics model $\ff_{t+1}$. Finally, the updated full state $\xx_{t+1}$, excluding $q_{t+1}$, is used by the updated dynamics model $\ff_{t+1}$ for prediction. %This unrolling mechanism proves to be stable, as we show in Section \ref{sec:experiments}.

We evaluate our model on pushing tasks in two settings: 
\begin{itemize}
    \item Given $K$ objects in a workspace, the robot needs  to push each of them to their designated goal positions.
    \item Given a single object \todo{with a few obstacles??}, the robot needs to plan an obstacle-avoidance trajectory and push the object to the desired goal.
\end{itemize}


We apply our approach with model predictive control (MPC). Our model is unrolled forward with randomly sampled action sequences, and we evaluate each action sequence based on the Euclidean distance of the predicted end-location of the objects from desired 3D locations. We execute the first action of the best found action sequence and repeat the  process for a fixed time horizon $T$.


==> note_related.tex <==
\section{Related Work}
\label{sec:related}


. These  methods infer a low-dimensional state of the system  from a history of 2D images or 3D poinclouds \cite{li2018push, xu2019densephysnet, DBLP:journals/corr/FinnL16, agrawal2016learning} and predict a representation for the sensory input for the next time step,  such as a future 2D image \cite{DBLP:journals/corr/FinnGL16,DBLP:journals/corr/FinnL16,ebert2018visual,actionconditioned,DBLP:journals/corr/abs-1710-05268,NIPS2015_5859,DBLP:journals/corr/abs-1903-00374}, image embedding from which an image will be reconstructed \cite{hafner2019planet}, object 2D locations from which a future image can be rendered \cite{DBLP:journals/corr/abs-1812-10972,Fragkiadaki2015LearningVP}. In the state inferred there is no explicit separation of static and dynamic properties. 

\paragraph{Model learning and model adaptation}
Learning dynamics  models that can generalise across environment physical and visual variations  is an open research problem whose solution would revolutionize model-based reinforcement learning, the field that investigates action selection by temporal unrolling of dynamics \cite{robotcontrol}. 
%Learning models of dynamics is a central research problem in machine learning and control. 
The difficulty of traditional analytical models to capture the complexity of real world systems \cite{} has led many researchers to pursue learning-based models of dynamics \citep{watter2015embed, banijamali2018robust, hafner2019planet, zhang2019solar}, or combine such models with analytic ones \citep{zeng2019tossingbot,ajay}. % to help the latter fight under-modeling and improve generalization. 


%Many works do not consider potential change in the underlying dynamics \cite{watter2015embed, banijamali2018robust, Fragkiadaki2015LearningVP,   zhang2019solar, hafner2019planet}, resulting in potential model in case of any changes in the system behavior. In order to account for varying dynamics, various approaches propose to learn dynamics models conditioning on system properties \cite{chen2018hardware, li2018learning, graphnet}. In the context of modeling interactions with objects, many works condition on 2D visual inputs \cite{DBLP:journals/corr/FinnL16,agrawal2016learning, li2018push,xu2019densephysnet, battaglia2016interaction}, hoping that the visual inputs capture both the state and properties of the system. This includes methods that predict dynamics in a 2D image space, such as future visual frames \citep{DBLP:journals/corr/MathieuCL15,actionconditioned,DBLP:journals/corr/FinnGL16,DBLP:journals/corr/abs-1812-00568}, neural encodings of future frames \citep{DBLP:journals/corr/abs-1803-10122,DBLP:journals/corr/ChiappaRWM17,hafner2019planet,agrawal2016learning,DBLP:journals/corr/PathakAED17}, object 2D motion trajectories \citep{Fragkiadaki2015LearningVP,DBLP:journals/corr/BattagliaPLRK16,DBLP:journals/corr/ChangUTT16}, and 2D pixel motion fields \citep{DBLP:journals/corr/FinnL16,DBLP:journals/corr/abs-1710-05268,DBLP:journals/corr/FinnGL16,SE3-Nets}.
%The last two sets of methods provide future visual observations during model unrolling by warping image pixels to generate future visual observations, and feed them into their model.
These methods use a single global model that takes system properties as input directly, together with its state and actions given by the agent. To infer implicit properties that can not be inferred from visual features, some works propose to encode a history of interactions with objects to infer their physics properties \cite{pushnet, densephysnet}.

For expressive dynamics models represented as neural networks, online adaptation via finetuning starting from some initial set of parameters is also explored. These approaches usually require many samples and multiple passes over the data to arrive at a sensible solution \citep{ijcai2018-369}.
For example, model agnostic meta-learning (MAML) \citep{DBLP:journals/corr/FinnAL17,Nagabandi2019LearningTA,clavera} learns a parameter initialization for a dynamics model which ought to generate a well adapted dynamics model with only a few interactions at test time.
Under diverse dynamic environments without some obvious similarity between them such an initialization learning approach has been found to require many samples to adapt effectively \citep{kaushik2020fast,DOMe}. The idea of using multiple model initializations for efficient adaptation to novel test conditions are investigated in \citep{adaptanimals,DOMe}.
\citet{kaushik2020fast} proposes dynamics models that alongside a state and action condition (through concatenation) on a situation embedding, which is jointly trained with a dynamics model.

\paragraph{Hyper-networks}
Central to HyperDynamics is the notion of using one network to generate the parameters of another network. 
This idea has previously been studied in various domains including image classification \citep{ha2016hypernetworks}, generative models \citep{ratzlaff2019hypergan}, and neural machine translation \citep{ha2016hypernetworks,platanios2018contextual}.
These works are motivated by various intuitions, such as using the structural features of the original network to generate network layers for reduction in the number of parameters \citep{ha2016hypernetworks}, generating an ensemble of networks for the same task to improve robustness to adversarial data \citep{ratzlaff2019hypergan}, or generating language encoders conditioned on the language context for better weight sharing across languages in a machine translation setting \citep{platanios2018contextual}.
To the best of our knowledge, this is the first work that applies the idea of generating model parameters to the domain of model-based RL, and proposes to generate expert models conditioned on system properties.


==> table_cap.tex <==

\begin{figure}[!t]
        \centering
        \tiny
        \sffamily
        \setlength{\tabcolsep}{3pt}
        \renewcommand{\arraystretch}{1.1}
        \captionof{table}{Prediction error of \textit{Direct} with varying model capacity.}
        \vspace{1ex}
        \begin{tabularx}{\textwidth}{|l||Y|Y|Y|Y|Y|Y|Y|Y|}
            \hhline{|-||-|-|-|-|-|-|-|-|}
            \textbf{Model}&
                        Ours & Direct  & Direct  & Direct   & Direct  & Direct  & Direct  & Direct  \\
            \hhline{:=::=:=:=:=:=:=:=:=:}
            Number of layers    & 4 & 4 &  8 & 16 & 64 & 4 &4 & 4 \\
            \hhline{|-||-|-|-|-|-|-|-|-|}
            Number of units per layer         & 32 & 32 & 32 & 32& 32  & 45 & 64 & 128 \\
            \hhline{|-||-|-|-|-|-|-|-|-|}
            Model capacity        & 16$\times$  & 1$\times$ & 2$\times$ & 4$\times$ & 16$\times$  & 2$\times$ & 4$\times$ & 16$\times$ \\
            \hhline{|-||-|-|-|-|-|-|-|-|}
            Prediction error (seen) & \best{0.83$\pm$0.35} & 1.01$\pm$0.41 & 0.98$\pm$0.46 & 1.19$\pm$0.51& 1.54$\pm$0.77& 0.98$\pm$0.41& 0.92$\pm$0.47& 0.86$\pm$0.34 \\
            \hhline{|-||-|-|-|-|-|-|-|-|}
            Prediction error (novel) & \best{0.93$\pm$0.53} & 1.24$\pm$0.54 & 1.25$\pm$0.50& 1.37$\pm$0.71& 1.87$\pm$0.89 & 1.26$\pm$0.62 & 1.33$\pm$0.61& 1.54$\pm$0.74\\
            \hhline{|-||--|--|--|--|}
        \end{tabularx}%
        
        \label{table:cap}
\end{figure}

